In-Place Rotation for Enhancing Snake-like Robot Mobility

Gaits engineered for snake-like robots to rotate in-place instrumentally fill a gap in the set of locomotive gaits that have traditionally prioritized translation. This paper designs a Turn-in-Place gait and demonstrates the ability of a shape-centric modeling framework to capture the gait's locomotive properties. Shape modeling for turning involves a time-varying continuous body curve described by a standing wave. Presumed viscous robot-ground frictional interactions lead to body dynamics conditioned on the time-varying shape model. The dynamic equations describing the Turn-in-Place gait are validated by an articulated snake-like robot using a physics-based simulator and a physical robot. The results affirm the shape-centric modeling framework's capacity to model a variety of snake-like robot gaits with fundamentally different body-ground contact patterns. As an applied demonstration, example locomotion scenarios partner the shape-centric Turn-in-Place gait with a Rectilinear gait for maneuvering through constrained environments based on a multi-modal locomotive planning strategy. Unified shape-centric modeling facilitates trajectory planning and tracking for a snake-like robot to successfully negotiate non-trivial obstacle configurations.

==> 14212206410/arxiv_submission/rl_ctrl2action_map_gz.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=7.233in,
height=1.413in,
at={(1.213in,5.062in)},
scale only axis,
xmin=-0.0015,
xmax=0.0015,
ymin=0,
ymax=50,
ylabel style={font=\color{white!15!black}},
ylabel={\LARGE $\bar{\xi}^b_x$ (mm/s)},
axis background/.style={fill=white},
every tick label/.append style={font=\Large},
xtick pos=left,
ytick pos=left,
%axis x line*=bottom,
%axis y line*=left,
%xmajorgrids,
%ymajorgrids
]
\addplot [color=blue, forget plot, line width=2.0pt]
  table[row sep=crcr]{%
-0.0015	36.0541956595813\\
-0.00146969696969697	36.0541956595813\\
-0.00143939393939394	36.0541956595813\\
-0.00140909090909091	36.0541956595813\\
-0.00137878787878788	36.0541956595813\\
-0.00134848484848485	36.0541956595813\\
-0.00131818181818182	36.0541956595813\\
-0.00128787878787879	36.0541956595813\\
-0.00125757575757576	36.0541956595813\\
-0.00122727272727273	36.0541956595813\\
-0.0011969696969697	36.0541956595813\\
-0.00116666666666667	36.0541956595813\\
-0.00113636363636364	36.0541956595813\\
-0.00110606060606061	36.0541956595813\\
-0.00107575757575758	36.0541956595813\\
-0.00104545454545455	36.0541956595813\\
-0.00101515151515152	36.0541956595813\\
-0.000984848484848485	36.0541956595813\\
-0.000954545454545455	36.0541956595813\\
-0.000924242424242424	36.0541956595813\\
-0.000893939393939394	36.0541956595813\\
-0.000863636363636364	36.0541956595813\\
-0.000833333333333333	36.0541956595813\\
-0.000803030303030303	36.0541956595813\\
-0.000772727272727273	36.0541956595813\\
-0.000742424242424242	36.0541956595813\\
-0.000712121212121212	36.0541956595813\\
-0.000681818181818182	36.0541956595813\\
-0.000651515151515152	36.0541956595813\\
-0.000621212121212121	36.0541956595813\\
-0.000590909090909091	36.0541956595813\\
-0.000560606060606061	36.0541956595813\\
-0.00053030303030303	36.0541956595813\\
-0.0005	36.0541956595813\\
-0.00046969696969697	36.0541956595813\\
-0.000439393939393939	36.0541956595813\\
-0.000409090909090909	36.0541956595813\\
-0.000378787878787879	36.0541956595813\\
-0.000348484848484848	36.0541956595813\\
-0.000318181818181818	36.0541956595813\\
-0.000287878787878788	36.0541956595813\\
-0.000257575757575758	36.0541956595813\\
-0.000227272727272727	36.0541956595813\\
-0.000196969696969697	36.0541956595813\\
-0.000166666666666667	36.0541956595813\\
-0.000136363636363636	36.0541956595813\\
-0.000106060606060606	36.0541956595813\\
-7.57575757575758e-05	36.0541956595813\\
-4.54545454545455e-05	36.0541956595813\\
-1.51515151515152e-05	36.0541956595813\\
1.51515151515152e-05	36.0541956595813\\
4.54545454545455e-05	36.0541956595813\\
7.57575757575758e-05	36.0541956595813\\
0.000106060606060606	36.0541956595813\\
0.000136363636363636	36.0541956595813\\
0.000166666666666667	36.0541956595813\\
0.000196969696969697	36.0541956595813\\
0.000227272727272727	36.0541956595813\\
0.000257575757575758	36.0541956595813\\
0.000287878787878788	36.0541956595813\\
0.000318181818181818	36.0541956595813\\
0.000348484848484848	36.0541956595813\\
0.000378787878787879	36.0541956595813\\
0.000409090909090909	36.0541956595813\\
0.000439393939393939	36.0541956595813\\
0.00046969696969697	36.0541956595813\\
0.0005	36.0541956595813\\
0.00053030303030303	36.0541956595813\\
0.000560606060606061	36.0541956595813\\
0.000590909090909091	36.0541956595813\\
0.000621212121212121	36.0541956595813\\
0.000651515151515152	36.0541956595813\\
0.000681818181818182	36.0541956595813\\
0.000712121212121212	36.0541956595813\\
0.000742424242424242	36.0541956595813\\
0.000772727272727273	36.0541956595813\\
0.000803030303030303	36.0541956595813\\
0.000833333333333333	36.0541956595813\\
0.000863636363636364	36.0541956595813\\
0.000893939393939394	36.0541956595813\\
0.000924242424242424	36.0541956595813\\
0.000954545454545455	36.0541956595813\\
0.000984848484848485	36.0541956595813\\
0.00101515151515152	36.0541956595813\\
0.00104545454545455	36.0541956595813\\
0.00107575757575758	36.0541956595813\\
0.00110606060606061	36.0541956595813\\
0.00113636363636364	36.0541956595813\\
0.00116666666666667	36.0541956595813\\
0.0011969696969697	36.0541956595813\\
0.00122727272727273	36.0541956595813\\
0.00125757575757576	36.0541956595813\\
0.00128787878787879	36.0541956595813\\
0.00131818181818182	36.0541956595813\\
0.00134848484848485	36.0541956595813\\
0.00137878787878788	36.0541956595813\\
0.00140909090909091	36.0541956595813\\
0.00143939393939394	36.0541956595813\\
0.00146969696969697	36.0541956595813\\
0.0015	36.0541956595813\\
};
\addplot[only marks, mark=*, mark options={}, mark size=3.0000pt, draw=red, fill=red, forget plot] table[row sep=crcr]{%
x	y\\
-0.0015	37.4571204291509\\
-0.001	37.1320600132173\\
-0.0005	34.3908352681062\\
1e-06	35.2929271840696\\
0.0005	36.8981969530268\\
0.001	37.099694032408\\
0.0015	34.1085357370901\\
};
\end{axis}

\begin{axis}[%
width=7.233in,
height=1.413in,
at={(1.213in,2.965in)},
scale only axis,
xmin=-0.0015,
xmax=0.0015,
ymin=-10,
ymax=10,
ylabel style={font=\color{white!15!black}},
ylabel={\LARGE $\bar{\xi}^b_y$ (mm/s)},
axis background/.style={fill=white},
every tick label/.append style={font=\Large},
xtick pos=left,
ytick pos=left,
%axis x line*=bottom,
%axis y line*=left,
%xmajorgrids,
%ymajorgrids
]
\addplot [color=blue, forget plot, line width=2.0pt]
  table[row sep=crcr]{%
-0.0015	0.105158318731939\\
-0.00146969696969697	0.105158318731939\\
-0.00143939393939394	0.105158318731939\\
-0.00140909090909091	0.105158318731939\\
-0.00137878787878788	0.105158318731939\\
-0.00134848484848485	0.105158318731939\\
-0.00131818181818182	0.105158318731939\\
-0.00128787878787879	0.105158318731939\\
-0.00125757575757576	0.105158318731939\\
-0.00122727272727273	0.105158318731939\\
-0.0011969696969697	0.105158318731939\\
-0.00116666666666667	0.105158318731939\\
-0.00113636363636364	0.105158318731939\\
-0.00110606060606061	0.105158318731939\\
-0.00107575757575758	0.105158318731939\\
-0.00104545454545455	0.105158318731939\\
-0.00101515151515152	0.105158318731939\\
-0.000984848484848485	0.105158318731939\\
-0.000954545454545455	0.105158318731939\\
-0.000924242424242424	0.105158318731939\\
-0.000893939393939394	0.105158318731939\\
-0.000863636363636364	0.105158318731939\\
-0.000833333333333333	0.105158318731939\\
-0.000803030303030303	0.105158318731939\\
-0.000772727272727273	0.105158318731939\\
-0.000742424242424242	0.105158318731939\\
-0.000712121212121212	0.105158318731939\\
-0.000681818181818182	0.105158318731939\\
-0.000651515151515152	0.105158318731939\\
-0.000621212121212121	0.105158318731939\\
-0.000590909090909091	0.105158318731939\\
-0.000560606060606061	0.105158318731939\\
-0.00053030303030303	0.105158318731939\\
-0.0005	0.105158318731939\\
-0.00046969696969697	0.105158318731939\\
-0.000439393939393939	0.105158318731939\\
-0.000409090909090909	0.105158318731939\\
-0.000378787878787879	0.105158318731939\\
-0.000348484848484848	0.105158318731939\\
-0.000318181818181818	0.105158318731939\\
-0.000287878787878788	0.105158318731939\\
-0.000257575757575758	0.105158318731939\\
-0.000227272727272727	0.105158318731939\\
-0.000196969696969697	0.105158318731939\\
-0.000166666666666667	0.105158318731939\\
-0.000136363636363636	0.105158318731939\\
-0.000106060606060606	0.105158318731939\\
-7.57575757575758e-05	0.105158318731939\\
-4.54545454545455e-05	0.105158318731939\\
-1.51515151515152e-05	0.105158318731939\\
1.51515151515152e-05	0.105158318731939\\
4.54545454545455e-05	0.105158318731939\\
7.57575757575758e-05	0.105158318731939\\
0.000106060606060606	0.105158318731939\\
0.000136363636363636	0.105158318731939\\
0.000166666666666667	0.105158318731939\\
0.000196969696969697	0.105158318731939\\
0.000227272727272727	0.105158318731939\\
0.000257575757575758	0.105158318731939\\
0.000287878787878788	0.105158318731939\\
0.000318181818181818	0.105158318731939\\
0.000348484848484848	0.105158318731939\\
0.000378787878787879	0.105158318731939\\
0.000409090909090909	0.105158318731939\\
0.000439393939393939	0.105158318731939\\
0.00046969696969697	0.105158318731939\\
0.0005	0.105158318731939\\
0.00053030303030303	0.105158318731939\\
0.000560606060606061	0.105158318731939\\
0.000590909090909091	0.105158318731939\\
0.000621212121212121	0.105158318731939\\
0.000651515151515152	0.105158318731939\\
0.000681818181818182	0.105158318731939\\
0.000712121212121212	0.105158318731939\\
0.000742424242424242	0.105158318731939\\
0.000772727272727273	0.105158318731939\\
0.000803030303030303	0.105158318731939\\
0.000833333333333333	0.105158318731939\\
0.000863636363636364	0.105158318731939\\
0.000893939393939394	0.105158318731939\\
0.000924242424242424	0.105158318731939\\
0.000954545454545455	0.105158318731939\\
0.000984848484848485	0.105158318731939\\
0.00101515151515152	0.105158318731939\\
0.00104545454545455	0.105158318731939\\
0.00107575757575758	0.105158318731939\\
0.00110606060606061	0.105158318731939\\
0.00113636363636364	0.105158318731939\\
0.00116666666666667	0.105158318731939\\
0.0011969696969697	0.105158318731939\\
0.00122727272727273	0.105158318731939\\
0.00125757575757576	0.105158318731939\\
0.00128787878787879	0.105158318731939\\
0.00131818181818182	0.105158318731939\\
0.00134848484848485	0.105158318731939\\
0.00137878787878788	0.105158318731939\\
0.00140909090909091	0.105158318731939\\
0.00143939393939394	0.105158318731939\\
0.00146969696969697	0.105158318731939\\
0.0015	0.105158318731939\\
};
\addplot[only marks, mark=*, mark options={}, mark size=3.0000pt, draw=red, fill=red, forget plot] table[row sep=crcr]{%
x	y\\
-0.0015	3.35092902569231\\
-0.001	1.67694734871943\\
-0.0005	2.77098387178409\\
1e-06	0.545709921608065\\
0.0005	-3.62441736068229\\
0.001	-0.455966458833062\\
0.0015	-3.52807811716496\\
};
\end{axis}

\begin{axis}[%
width=7.233in,
height=1.413in,
at={(1.213in,0.867in)},
scale only axis,
xmin=-0.0015,
xmax=0.0015,
xlabel style={font=\color{white!15!black}},
xlabel={\LARGE $\kappa$ (mm$^{-1}$)},
ymin=-10,
ymax=10,
ylabel style={font=\color{white!15!black}},
ylabel={\LARGE $\bar{\xi}^b_\omega$ (deg/s)},
axis background/.style={fill=white},
every tick label/.append style={font=\Large},
xtick pos=left,
ytick pos=left,
%axis x line*=bottom,
%axis y line*=left,
%xmajorgrids,
%ymajorgrids
]
\addplot [color=blue, forget plot, line width=2.0pt]
  table[row sep=crcr]{%
-0.0015	2.50399191927549\\
-0.00146969696969697	2.45257663714607\\
-0.00143939393939394	2.40116135501664\\
-0.00140909090909091	2.34974607288721\\
-0.00137878787878788	2.29833079075779\\
-0.00134848484848485	2.24691550862836\\
-0.00131818181818182	2.19550022649893\\
-0.00128787878787879	2.1440849443695\\
-0.00125757575757576	2.09266966224008\\
-0.00122727272727273	2.04125438011065\\
-0.0011969696969697	1.98983909798122\\
-0.00116666666666667	1.93842381585179\\
-0.00113636363636364	1.88700853372237\\
-0.00110606060606061	1.83559325159294\\
-0.00107575757575758	1.78417796946351\\
-0.00104545454545455	1.73276268733408\\
-0.00101515151515152	1.68134740520466\\
-0.000984848484848485	1.62993212307523\\
-0.000954545454545455	1.5785168409458\\
-0.000924242424242424	1.52710155881637\\
-0.000893939393939394	1.47568627668695\\
-0.000863636363636364	1.42427099455752\\
-0.000833333333333333	1.37285571242809\\
-0.000803030303030303	1.32144043029867\\
-0.000772727272727273	1.27002514816924\\
-0.000742424242424242	1.21860986603981\\
-0.000712121212121212	1.16719458391038\\
-0.000681818181818182	1.11577930178096\\
-0.000651515151515152	1.06436401965153\\
-0.000621212121212121	1.0129487375221\\
-0.000590909090909091	0.961533455392674\\
-0.000560606060606061	0.910118173263247\\
-0.00053030303030303	0.85870289113382\\
-0.0005	0.807287609004392\\
-0.00046969696969697	0.755872326874965\\
-0.000439393939393939	0.704457044745537\\
-0.000409090909090909	0.65304176261611\\
-0.000378787878787879	0.601626480486683\\
-0.000348484848484848	0.550211198357255\\
-0.000318181818181818	0.498795916227828\\
-0.000287878787878788	0.447380634098401\\
-0.000257575757575758	0.395965351968973\\
-0.000227272727272727	0.344550069839546\\
-0.000196969696969697	0.293134787710119\\
-0.000166666666666667	0.241719505580691\\
-0.000136363636363636	0.190304223451264\\
-0.000106060606060606	0.138888941321836\\
-7.57575757575758e-05	0.0874736591924091\\
-4.54545454545455e-05	0.0360583770629818\\
-1.51515151515152e-05	-0.0153569050664456\\
1.51515151515152e-05	-0.066772187195873\\
4.54545454545455e-05	-0.1181874693253\\
7.57575757575758e-05	-0.169602751454728\\
0.000106060606060606	-0.221018033584155\\
0.000136363636363636	-0.272433315713582\\
0.000166666666666667	-0.32384859784301\\
0.000196969696969697	-0.375263879972437\\
0.000227272727272727	-0.426679162101864\\
0.000257575757575758	-0.478094444231292\\
0.000287878787878788	-0.529509726360719\\
0.000318181818181818	-0.580925008490146\\
0.000348484848484848	-0.632340290619574\\
0.000378787878787879	-0.683755572749001\\
0.000409090909090909	-0.735170854878428\\
0.000439393939393939	-0.786586137007856\\
0.00046969696969697	-0.838001419137283\\
0.0005	-0.889416701266711\\
0.00053030303030303	-0.940831983396138\\
0.000560606060606061	-0.992247265525565\\
0.000590909090909091	-1.04366254765499\\
0.000621212121212121	-1.09507782978442\\
0.000651515151515152	-1.14649311191385\\
0.000681818181818182	-1.19790839404327\\
0.000712121212121212	-1.2493236761727\\
0.000742424242424242	-1.30073895830213\\
0.000772727272727273	-1.35215424043156\\
0.000803030303030303	-1.40356952256098\\
0.000833333333333333	-1.45498480469041\\
0.000863636363636364	-1.50640008681984\\
0.000893939393939394	-1.55781536894927\\
0.000924242424242424	-1.60923065107869\\
0.000954545454545455	-1.66064593320812\\
0.000984848484848485	-1.71206121533755\\
0.00101515151515152	-1.76347649746698\\
0.00104545454545455	-1.8148917795964\\
0.00107575757575758	-1.86630706172583\\
0.00110606060606061	-1.91772234385526\\
0.00113636363636364	-1.96913762598469\\
0.00116666666666667	-2.02055290811411\\
0.0011969696969697	-2.07196819024354\\
0.00122727272727273	-2.12338347237297\\
0.00125757575757576	-2.17479875450239\\
0.00128787878787879	-2.22621403663182\\
0.00131818181818182	-2.27762931876125\\
0.00134848484848485	-2.32904460089068\\
0.00137878787878788	-2.3804598830201\\
0.00140909090909091	-2.43187516514953\\
0.00143939393939394	-2.48329044727896\\
0.00146969696969697	-2.53470572940839\\
0.0015	-2.58612101153781\\
};
\addplot[only marks, mark=*, mark options={}, mark size=3.0000pt, draw=red, fill=red, forget plot] table[row sep=crcr]{%
x	y\\
-0.0015	2.70590222823811\\
-0.001	1.36401938782279\\
-0.0005	0.69061778929647\\
1e-06	0.0531182983844796\\
0.0005	-0.597078745569514\\
0.001	-1.896572348535\\
0.0015	-2.60915513686573\\
};
\end{axis}
\end{tikzpicture}%


==> 14212206552/arxiv_submission/conclusion.tex <==
%\color{red}
%Comparison of Gazebo simulation results with physical simulation, here, also serve to validate outcomes presented in Section \secref{results}, where experiments entail larger-scale locomotion scenarios that are easier to manage in simulation, than physical experiment.
%\color{black}

The paper described Turn-in-Place gait for snake-like robots, whose
standing wave and body-contact properties were engineered to primarily
produce net rotational motion. The rigid dynamics of the body frame were
derived using a shape-centric modeling framework
\cite{ChVe_RAS[2020]} with viscous body-ground friction.
Validation of the resulting integro-differential dynamical equations
employed the Gazebo simulator and physical experiments for a $12$-link
articulated robot.

The Turn-in-Place gait is the fourth motion primitive whose evolution
the shape-centric modeling approach is capable of describing. It is
further evidence that the framework constitutes a unified modeling
approach for describing the locomotive behavior of a variety of
gaits for snake-like robots.  In characterizing each gait's
time-averaged movement, we obtain a reduced-order control-to-action map
describing each gait's steady-state locomotive behavior as a function of
its input shape parameters. The maps resemble unicycle-like motion
profiles such that planning and control frameworks commonly used for
differential-drive vehicles apply to the snake-like robot.  Pairing the
Turn-in-Place gait with a previously modeled Rectilinear gait in a
multi-gait planning and tracking strategy permits traversal through
environments requiring high angular displacements.  The snake-like robot
successfully tracks multi-gait trajectory plans, in Gazebo simulation,
to complete several navigation scenerios.
%Only together, are the gaits able to accomplish each obstacle scenario.

The Turn-in-Place gait fills a critical gap in the space of motion
profiles achievable by snake-like robots. The utility of rotating
in-place is evident in the locomotion scenarios demonstrated here. By
filling this mobility gap, a greater breadth of planning and tracking
control approaches, commonly used for differential-drive vehicles,
become applicable for snake-like robot locomotion.  Future work aims to
replicate the simulations on the physical robot, once a means to track
its pose over long distances has been established.



==> 14212206571/arxiv_submission/intro.tex <==
%Principal locomotion objectives, for mobile robots, typically entail moving the robot's body frame from one geographic position to another, e.g. in $E(2)$. 
Gait-based snake-like robot locomotion over flat ground has primarily
focused on a handful of motion primitives: lateral undulation,
sidewinding and rectilinear forms of motion. These gaits exhibit
predominantly-translational movement.
In application, they are used by snake-like robots to achieve large
translational displacements (many body lengths) to reach prescribed goal
positions. Steering during locomotion involves modulating gait parameters
to induce steering effects
\cite{KoEtAl_BnB[2016], YaWaSh_AIM[2019], AsEtAl_PNAS[2015],
XiEtAl_ICRA[2015], ChVe_RAS[2020]}. For lateral undulation and rectilinear
gaits, steering relies on joint offsets. For conical sidewinding, the  
cone half-angle mediates the turning rate.
The steering parameters govern the robot's body shape during locomotion
and are subject to saturation limits. Beyond the limits, the prescribed
body shape is not realizable, either due to actuator constraints or
due to self-collision.  Consequently, the curved trajectories resulting
from these gaits are similarly subject to a saturating turning rate.
There is a limit to how tightly the robot may turn under
translation-dominant gaits. 

Locomotive models for translational gaits have been derived as either
dynamic or kinematic motion models. Derivations of lateral undulation
and rectilinear models are specialized to the particular gait
of interest and to the underlying snake-like robot design 
\cite{LiEtAl_Springer[2013],TaReMa_IROS[2015],TaMa_ICRA[2015]}. 
Follow-on trajectory control strategies are tied to the particular
gait's motion model, possibly with provable tracking guarantees
\cite{LiEtAl_Springer[2013]}. Conical forms of sidewinding have been
studied under the presumption of ideally-static rolling body-ground
contact. A kinematic analysis results in a closed-form motion model,
parametrized with respect to the gait's input shape parameters
\cite{GoEtAl_ICRA[2012]}. A re-parametrization allows this gait to be
re-framed as a simple differential-drive vehicle, for which traditional
path tracking approaches may then be applied \cite{XiEtAl_ICRA[2015]}.
Alternatively, a shape-centric modeling framework has been presented,
whereby shape kinematics and locomotive dynamics of various bio-inspired
gaits for snake-like robots are described through a unified modeling
approach \cite{ChVe_RAS[2020], ChSeVe_CDC[2016b]}.
Reduced-order motion models, that capture the time-averaged kinematic
behavior of each gait, can be empirically-derived from the full system
dynamics. Reduction of complex dynamics associated with snake-like
robotic gaits, to simplified motion models, facilitates locomotive
planning and control \cite{ChVe_RAS[2020], ChEtAl_ACC[2018]}. 
This model reduction approach realizes the framework proposed in
\cite{McOs_IJRR[2003]}. 
%Gaits may be successively reduced to unicycle-like vehicles, where non-zero linear velocities produce curved trajectories in the plane of locomotion. 
An attractive property of the shape-centric modeling framework is its
ability describe a variety of gaits and to produce uniformly structured
motion models for each. Planning and control strategies 
viable for one gait apply to other gaits modeled using this approach.
This generalization is meaningful for snake-like robots, and potentially
other bio-inspired robots; organisms that serve as bio-inspirational
focus frequently exhibit several modes of locomotion to accommodate
varying environmental situations \cite{LoEtAl_BnB[2010],LoEtAl_BnB[2015]}. 

More recently, gaits for elongated-body, limbless robots have been
designed that `rotate-in-place'. While no known snake species exhibit
gaits that accomplish this motion profile, biological inspiration has
been found in nematode worms, a different elongated-body and limbless
organism \cite{WaEtAl_IROS[2020]}. A turn-in-place gait variant,
designated `frequency turning', has been discovered through an empirical
search through the robot shape space \cite{GoEtAl_ICRA[2015], AsEtAl_PNAS[2015]}. 
The net change in orientation achieved over a single cycle of these gaits 
is large, while net translation remains relatively small. 
Interestingly, the nematode worm-inspired Omega Turn relies solely on
planar shape changes, with no vertical lift, to accomplish rotation;
the latter frequency turning gait instead accomplishes this through
strategic body-ground contact planning. Motion models for these gaits
are grounded in the articulated platforms on which they are applied and
involve elements of empirical sampling for different locomotion
environments.

The unique motion profile characterizing turn-in-place gaits fills an important 
gap in the space of locomotive behaviors available to snake-like robots. 
Additing a turn-in-place gait to their toolbox realizes the ability to
mimic differential-drive wheeled robots. 
As a consequence, planning and tracking control approaches frequently
used on wheeled robots become more comprehensively applicable to
snake-like robots.  These wheeled platforms can steer while commanding
non-zero linear velocities, and can arbitrarily re-orient in-place at
(near) zero linear velocity.  In a similar manner, multi-modal switching
between turn-in-place and translationally-focused gaits permit
snake-like robots to traverse paths that neither gait alone may achieve.
This greatly broadens set of navegable locomotion scenarios for
snake-like robots, as candidate trajectory solutions are no longer
constrained by turning rate limits.
%Predominantly-translational gaits produce trajectories limited by a maximum curvature; strategic swapping with a turn-in-place gait overcomes this limitation at the expense of translational progress (i.e. time). 

%Multi-modal motion planning is a common challenge in several fields of robotics, where a finite, discrete set of motion primitives must strategically sequenced and controlled to accomplish an objective. For mobile soft robots, permutated sequences of body shape maneuvers lead to a large set of gaits \cite{ViGrTr_IROS[2015], WaWaFe_TMech[2021]}; locomotive planning involves an optimization search over the space of feasible gait sequences. 
%In service robotics, this challenge may involve optimization over feasible sequences of continuously-parametrized manipulator actions, in addition to transit of the robot itself \cite{HaHiGo_IJRR[2011], DoEtAl_ICRA[2018]}. 

\noindent {\bf Contribution.}
We design a Turn-in-Place gait for snake-like robots with standing wave
shape kinematics. A shape-centric modeling framework
\cite{ChVe_RAS[2020]} conditioned on the gait describes the robot's locomotive
dynamics. 
The gait is represented by a time-varying continuous body curve defined
with respect to a static average body reference curve and rigid body frame. 
Planar group dynamics are derived for this continuous-body gait after
introducing a strategically-engineered body-ground contact pattern and
using a viscous friction model. 
The equations of motion are validated in a physics-based simulator
(Gazebo) and on a physical snake-like robot.
%
The validation highlights the shape-centric modeling framework's
capacity to describe a variety of snake-like robot gaits in a unified
manner. The uniformly-structured gait models that result are useful in
locomotion planning and control.  
%
Integrated use of the Turn-in-Place gait with a pre-existing Rectilinear gait 
leads to a multi-gait trajectory synthesis and tracking strategy.
A snake-like robot can then traverse obstacle-strewn scenarios requiring
tight turns by exploiting each gait's affordances.





==> 14212206571/arxiv_submission/plan_track.tex <==
Multi-gait trajectory synthesis is accomplished using a three-pass
approach to output a discrete-time reference trajectory with
feed-forward controls.  Each pass after the first incrementally refines
the current trajectory.  The final product is a controlled,
switched-gait trajectory designed to move the robot from its starting
pose to a prescribed goal position.  Synthesis is specialized to the two
gaits, Rectilinear and Turn-in-Place, $\mathcal{MP} = \{ {\rm RL}, {\rm
TiP} \}$.  The Rectilinear gait employs a caterpillar-like,
anteriorly-propagating body wave to produce (predominantly)
translational motion. Limited turning ability is accomplished by
modulating the average (reference) body curvature $\kappa$
\cite{ChVe_RAS[2020]}. Its control-to-action map in the Gazebo
simulation environment is, 
\begin{equation} \eqlabel{control_to_action_map_RL}
  \bm{\Phi}^{\rm RL}(\kappa) = \mymatrix{36 \text{ mm/s}, 0 \text{ mm/s}, \text{-}1696.7 \hspace{-1pt} \cdot \hspace{-1pt} \kappa \text{ deg/s}}^T, 
\end{equation}
for $\kappa \in \left[ -1.5e\text{-}3, 1.5e\text{-}3 \right]$ mm$^{-1}$. Other gait parameters associated with the Rectilinear gait remain fixed: frequency ($f^{\rm RL} = -0.4$ Hz), body wave amplitude ($A^{\rm RL} = 60$ mm), wavelength ($\lambda^{\rm RL} = 390$ mm).
The Turn-in-Place control-to-action map is \eqref{cntrl2action_TiP}. 
The map captures locomotive behavior as a kinematic motion model,
parametrized with respect to peak amplitude $\bar{A}$.

Trajectory synthesis starts with a collision-free input seed path
$\bm{G}^{\rm seed}$ consisting of a sequence of coordinates connecting
the robot's start pose and goal position, typically generated using
one's traditional path planning approach \cite{Latombe_RoboMP[1991]}
of choice.  The path generated in this first pass is absent of any
control or timing information and is not constrained by the robot's
locomotive dynamics. 

\subsection{Pass 2: Unicycle-based Trajectory Synthesis}
\seclabel{MPC_traj_synth}
Pass 2 parametrizes the path $\bm{G}^{\rm seed}$ with respect to time.
Presuming a fixed arc length speed consistent with the Rectilinear gait,
the path is re-sampled at a fixed number of Rectilinear gait periods,
$T^{\rm intvl} = \bar{N}^{\rm RL}/{f^{\rm RL}}$, where $\bar{N}^{\rm RL}
= 2$. 
%
This discrete-time path is the reference path for a model predictive
control (MPC) output tracker based on a unicycle motion model whose
inputs are linear and angular velocities, $v^{\rm uni}$ and $\omega^{\rm uni}$.
Additional constraints limit the unicycle model to motion that is
collectively achievable by the gaits in $\mathcal{MP}$,
\begin{equation}
v^{\rm uni} \in \left[ \Phi^{\rm RL}_x(\kappa) - \epsilon, \Phi^{\rm
RL}_x(\kappa) + \epsilon \right]\ \land\  
\omega^{\rm uni} \in \left[ \omega^{\rm TiP}_{\rm min}, \ \omega^{\rm TiP}_{\rm max} \right]
\end{equation}
%\begin{align}
%v^{\rm uni} &\in \left[ \Phi^{\rm RL}_x(\kappa) - \epsilon, \Phi^{\rm RL}_x(\kappa) + \epsilon \right], \\
%\omega^{\rm uni} &\in \left[ \omega^{\rm TiP}_{\rm min}, \ \omega^{\rm TiP}_{\rm max} \right],
%\end{align}
where
\begin{equation}
\omega^{\rm TiP}_{\rm min} = \min_{\bar{A}}\Phi^{\rm TiP}_\omega \left(
\bar{A} \right)\ \text{and}\ 
\omega^{\rm TiP}_{\rm max} = \max_{\bar{A}} \Phi^{\rm TiP}_\omega \left( \bar{A} \right).
\end{equation}
The small constant $\epsilon$ adds slack to assist with convergence to a
solution. In summary, linear velocity is constrained to that achievable
by the Rectilinear gait, while the Turn-in-Place gait defines allowable
angular velocities.

The output is 
$\left( \bm{G}^{\rm uni}, \bm{t}^{\rm uni}, \bm{U}^{\rm uni} \right)$,
a collection of sets each of which has cardinality $N^{\rm uni}$.
$\bm{G}^{\rm uni} = \left\{ g^{\rm uni}_i \in SE(2) \right\}^{N^{\rm
uni}}_{i = 1}$ is a sequence of pose coordinates. 
A corresponding time schedule $\bm{t}^{\rm uni}$ consists of timestamps
at intervals of $T^{\rm intvl}$ seconds. 
Lastly, $\bm{U}^{\rm uni} = \left\{ \left( v^{\rm uni}_i, w^{\rm uni}_i
\right) \right\}^{N^{\rm uni}}_{i = 1}$ are the open-loop control
inputs for achieving the pose sequence $\bm{G}^{\rm uni}$. 

\subsection{Pass 3: Multi-gait Refinement}
Pass 3 further revises the sets based on which gaits in $\mathcal{MP}$
will realize the desired displacements.
Stepping through each trajectory point $i = 1 \ldots
N^{\rm uni}$, the ability of the Rectilinear gait to apply the
associated open-loop control is tested:
\begin{equation} \eqlabel{w_thresh_RL_TiP}
  {\rm isRLTraversable}(i) = \left( \omega^{\rm uni}_i \leq 0.85 \cdot \omega^{\rm RL}_{\rm max} \right) \\
\end{equation}
for the maximum angular velocity of the Rectilinear gait,
\begin{equation}
  \omega^{\rm RL}_{\rm max} = \max_{\kappa} \Phi^{\rm RL}_\omega \left( \kappa \right).
\end{equation}
Trajectory points satisfying \eqref{w_thresh_RL_TiP} entail feasible angular
velocities $\omega^{\rm uni}_i$ for the Rectilinear gait using
an average (reference) body curvature
$\kappa_i = \left(\Phi^{\rm RL}_\omega \right)^{-1} \left(\omega^{\rm uni}_i\right)$. 

Trajectory segments where \eqref{w_thresh_RL_TiP} is false are presumed
infeasible for the Rectilinear gait. The robot will employ a
Turn-in-Place, Rectilinear, Turn-in-Place gait sequence to negotiate
them. A trajectory segment \textit{not} satisfying \eqref{w_thresh_RL_TiP}, beginning at point $j$ and ending at point $k > j$, is circumvented by connecting a straight line between the two points; we denote this line's spatial orientation as $\theta_{j \rightarrow k}$. At point $j$, a series of $6$ Turn-in-Place gait cycles (trajectory points) is inserted to close the error, $\theta_{j \rightarrow k} - \theta^{\rm uni}_{j}$, with an angular velocity $\omega^{\rm MG} = \frac{(\theta_{j \rightarrow k} - \theta^{\rm uni}_{j}) \cdot f^{\rm TiP}}{6}$. Following this, we insert a series of Rectilinear gait cycles to traverse the distance from $g^{\rm uni}_{j}$ to $g^{\rm uni}_k$, with the Rectilinear turning parameter fixed to $\kappa = 0$; the number of Rectilinear gait cycles inserted is dictated by the fixed speed at which the gait travels, $\Phi^{\rm RL}_x(\kappa)$. 
At $g^{\rm uni}_k$, a final sequence of $6$ Turn-in-Place gait cycles is inserted to close the remaining orientation error, $\theta^{\rm uni}_{k} - \theta_{j \rightarrow k}$, with angular velocity $\omega^{\rm MG} = \frac{(\theta^{\rm uni}_{k} - \theta_{j \rightarrow k}) \cdot f^{\rm TiP}}{6}$. Turn-in-Place input parameters needed to achieve a desired angular velocity are $\bar{A} = \left( \Phi^{\rm TiP}_\omega \right)^{-1} \left(\omega\right)$.
%In lieu of following trajectory segments requiring large angular velocities, we opt to instead `cut' these sharper corners. 

The refined multi-gait trajectory is described by the collection, $\left( \bm{G}^{\rm MG}, \bm{t}^{\rm MG}, \bm{M\!P}^{\rm MG}, \bm{U}^{\rm MG} \right)$. Each set in the collection is of cardinality $N^{\rm MG}$, the total number of points in the refined multi-gait trajectory. $\bm{G}^{\rm MG}$ and $\bm{t}^{\rm MG}$ denote planned pose coordinates and time, respectively. $\bm{M\!P}^{\rm MG} = \left\{ mp^{\rm MG}_i \in \mathcal{MP} \right\}^{N^{\rm MG}}_{i=1}$ expresses the gait sequence designed to traverse $\bm{G}^{\rm MG}$, while $\bm{U}^{\rm MG} = \left\{ \beta^{\rm MG}_i \in \mathbb{R} \right\}^{N^{\rm MG}}_{i=1}$ contains the gait-specific input parameter to be commanded at each trajectory point. $\beta^{\rm MG}_i$ describes either Rectilinear curvature $\kappa^{\rm MG}_i$ or Turn-in-Place peak amplitude $\bar{A}^{\rm MG}_i$, when $mp^{\rm MG}_i = \text{RL or TiP}$, respectively.

\subsection{Trajectory Tracking}
Tracking of the multi-gait trajectory is accomplished using simple
proportional feedback control. Feedback control is computed at scheduled
time intervals, specified in $\bm{t}^{\rm MG}$. We denote the waypoint
being tracked by its index $i = 1 \ldots N^{\rm MG}$. The pose error
associated with any waypoint $g^{\rm MG}_i \in \bm{G}^{\rm MG}$ and
robot pose $g$ is $g_{\rm err} = g^{-1} \cdot g^{\rm MG}_i$. It is the
the waypoint frame $g^{\rm MG}_i$ relative to the actual robot
frame. Individual translational and rotational errors, 
$\left( x_{\rm err}, y_{\rm err}, \theta_{\rm err} \right)$, are extracted.

Feedback-correction is dependent upon the planned gait $mp_{i}$, at a each waypoint $i$,
\begin{equation}
\omega_{\rm fb} = 
\begin{cases}
k^{\rm RL}_{\theta} \cdot \theta_{\rm err} + k^{\rm RL}_{y} \cdot y_{\rm err}, & mp_{i} = \text{RL} \\
k^{\rm TiP}_{\theta} \cdot \theta_{\rm err}, & mp_{i} = \text{TiP} 
\end{cases}.
\end{equation}
The open-loop gait parameter, $\kappa^{\rm MG}_i$ or $\bar{A}^{\rm
MG}_i$, is incorporated as a feed-forward value in the applied control,
\begin{align}
\kappa_{\rm fb} = \left( \Phi^{RL}_{\omega} \right)^{-1} \left( \Phi^{RL}_{\omega}\left( \kappa^{\rm MG}_{i} \right) + \omega_{\rm fb} \right), & \ mp_{i} = \text{RL} \\
\bar{A}_{\rm fb} =  \left( \Phi^{TiP}_{\omega} \right)^{-1} \left( \Phi^{TiP}_{\omega}\left( \bar{A}^{\rm MG}_i \right) + \omega_{\rm fb} \right), & \ mp_{i} = \text{TiP} 
\end{align}

As the robot proceeds sequentially through the planned waypoints, in $\bm{G}^{\rm MG}$, the forward error is assessed. If it exceeds a threshold, $x_{\rm err} > \bar{d}_{\rm err}$, the relevant target waypoint $i$ is \textit{not} incremented; the robot continues tracking the same waypoint until forward error falls below $\bar{d}_{\rm err}$.




==> 14212207532/arxiv_submission/tip_gait.tex <==
\begin{figure*} [!t]
\vspace{1.0mm}
\centering
  \begin{subfigure}{0.65\columnwidth}
  \centering
  \resizebox{1.0\columnwidth}{!}{\input{tip_gait_shape_1.tex}} 
	\caption{$t = 0$ sec.}
	\label{tip_gait_shape01}
	\end{subfigure}
	\hfill
  \begin{subfigure}{0.65\columnwidth}
  \centering
  \resizebox{1.0\columnwidth}{!}{\input{tip_gait_shape_2.tex}} 
	\caption{$t = 1.25$ sec.}
	\label{tip_gait_shape02}
	\end{subfigure}
	\hfill
  \begin{subfigure}{0.65\columnwidth}
  \centering
  \resizebox{1.0\columnwidth}{!}{\input{tip_gait_shape_3.tex}} 
	\caption{$t = 4.3$ sec.}
	\label{tip_gait_shape03}
	\end{subfigure}
	\caption{Sequence of Turn-in-Place gait shapes and component curves, over the course of one gait cycle ($T = 5$ sec.): reference body curve $\abProject(s, t)$ (dashed brown); planar body curve $\gSpace(s)$ (green+purple); body-ground contact segments $\mathcal{S}_{\rm cont}(t)$ (purple).} 
	\label{tip_gait_shape}
\end{figure*}


Recognizing the need for locomotion that goes beyond primarily
translational movement for snake-like robots has led to the design of
gaits with large angular and small translational displacements, 
i.e., turning in-place.  Such gaits complement the gaits traditionally
used for snake-like robot locomotion that achieve large translational
displacements to follow reference paths and reach goal positions many
body lengths distant. Two examples being the Omega Turn
as engineered from biologically-inspired observations of worms
\cite{WaEtAl_IROS[2020]}, and `frequency turning' as discovered
through a parameter sweep of a parametrized gait \cite{DaEtAl_ICRA[2015]}. 
Gait shapes associated with both are formulated as traveling waves and
vary in their use of vertical lift to manage body-ground contact. 
%
Here, we design a Turn-in-Place gait from basic physical principles. A
standing wave gait shape is coupled with a coordinated body-ground
contact profile to generate periodic stepping motion, whereby each step
rotates the snake in-place.  Modeling of the gait dynamics employs a
shape-centric modeling framework \cite{ChVe_RAS[2020]} to confirm
Turn-in-Place movement.

The full 3-D gait shape is represented by a continuous-body curve,
$\bCurvePos$, defined relative to a reference body curve, $\abCurvePos$,
and rigidly attached body frame.  Analysis of the gait's locomotive
properties focuses on the gait shape projection of $\bCurvePos$ onto the
plane of locomotion. This projected shape is denoted by $\gSpacePos$.
The component of $\bCurvePos$ describing vertical lifting of the body
from the ground will be described by a body-ground contact profile,
defined along $\gSpace(s, t)$.  Under this model, design of the
Turn-in-Place gait kinematics reduces to engineering a time-cyclical
body shape, $\gSpace(s, t)$, and a coordinated body-ground contact
profile $\mathcal{S}_{\rm cont}(t)$. 
%A body shape component that accomplishes vertical lift of the snake from the ground, may be reverse engineered from this contact pattern; the 3-D gait shape of the robot is recovered by superpositioning this with $\gSpace(s, t)$. 

\subsection{Gait Shape}
The Turn-in-Place gait shape description in the locomotion modeling plane, $\gSpacePos$, is a sinusoidal
standing wave; see Figure \ref{tip_gait_shape}. Its planar shape is
defined with respect to the reference body curve's projection onto the
locomotion plane, $\abProject(s, t)$. For this gait, $\abProject(s, t)$
is a straight line parametrized with respect to arc length, $s$. The
body frame $g \in SE(2)$ is rigidly attached to the reference body at
the center of the reference body where $s = 0$. The length of the
reference body is $L$ such that $s \in \left[ -\frac{L}{2}, \frac{L}{2}
\right]$. The Turn-in-Place gait standing wave is 
\begin{equation} \eqlabel{gait_shape}
  \gSpacePos = 
  \mymatrix{s \\ A(t) \sin \left( 2 \pi \cdot \frac{s}{\lambda(t)} \right)}
\end{equation}
where
\begin{equation} \eqlabel{gait_shape_Ah}
  A(t) = \bar{A} \sin(\pi f t) 
\end{equation}
for peak amplitude $\bar{A}$, frequency $f$ and corresponding gait
period  $T = \frac{1}{f}$.
The wavelength, $\lambda(t)$, is a function of $A(t)$ and the total
fixed curve length $\bar{L}$ (i.e., robot body length). 
It is computed by the root-finding operation, $\lambda(t) = {\rm
root}_{\gamma} \left( {\rm Arclen}\left( \gSpace(s, t; A(t), \gamma)
\right) - \bar{L} \right)$.  The gait is designed to be a single
sinusoidal standing wave, $L(t) = \lambda(t)$, periodic in time.
%\textcolor{red}{Note that the principle parameter defining the shape is $\bar{A}$; $A(t)$ and $\lambda(t)$ are prescribed functions, conditioned on $\bar{A}$ and $\bar{L}$.}

The robot begins each gait cycle in a straight-body configuration, illustrated in Figure \ref{tip_gait_shape01}, where $\gSpace(s, t)$ is denoted by the union of purple and green curve segments. Over the course of a half gait period, the shape transitions to a sine wave comprising a single wavelength, $\lambda$ (Fig. \ref{tip_gait_shape02}). During the second half of the gait cycle, this shape transitions back to a straight-body configuration (Fig. \ref{tip_gait_shape03}).

The rigid reference frame and the gait shape define a set of local
frames $\gshape(s, t) \in SE(2)$ residing along the body curve $\gSpace(s, t)$ 
whose local $x$-axis is tangent to the body curve. The frame decomposes
into a rotation, $R(s, t) \in SO(2)$, and a translation,
$\gSpace(s, t) \in E(2)$, specified relative to the rigid body frame, $g$. 

A vertical body curve component, $h(s, t)$, dictates which segments of the
body are in ground contact and when. It is constructed such that the segments in ground contact 
follow a desired contact schedule $\mathcal{S}_{\rm cont}(t)$, in \eqref{tip_contact}, for this gait.
The full 3-D gait shape is described as, $\bCurvePos = \gSpacePos + h(s, t)$.

\begin{figure*}[t]
  \centering
  \normalsize
  \begin{equation} \eqlabel{tip_contact}
    \mathcal{S}_{\rm cont}(t) = 
      \begin{cases}
        \left\{ s \in \left[-\frac{\ell_{\rm cont}}{2}, \frac{\ell_{\rm cont}}{2}\right] \cup \left[\frac{L}{2}-\frac{\ell_{\rm cont}}{2}, \frac{L}{2}+\frac{\ell_{\rm cont}}{2}\right] \right\} & t \in [0, \frac{T}{2}) \\
%
        \left\{ s \in \left[ -\frac{L}{2}, \frac{L}{2} \right] \right\} & t \in [\frac{T}{2}, T) 
      \end{cases}, 
      \text{where } \ell_{\rm cont}(t) = \max \left( \frac{L}{4} \left( 1+\cos\left(4 \pi f t\right) \right), \bar{\ell}_{\rm cont} \right)
    \end{equation}
  \hrulefill
  \vspace*{-0.8em}
\end{figure*}

\subsection{Robot-Environment Contact}
Vertical shape deformations of the snake-robot lead to desired
robot-ground interaction forces. 
%Vertical shape deformations of the snake-robot rely on the desired
%ground-robot interaction forces, which are dictated by what part of the
%body makes contact when. 
Here, the time-periodic body-ground contact
pattern is engineered to promote in-plane rotation through a stepping
pattern coupled to asymmetrical contact velocities.  In reference to
Figure \ref{tip_gait_shape}, body-ground contact segments are
illustrated as purple curves (green means no contact). 
The set of points along the body with ground contact is represented by 
\eqref{tip_contact}, where $\ell_{\rm cont}(t)$ denotes the
cyclically-varying length of each contact segment. Both contact segments
maintain a minimum length $\bar{\ell}_{\rm cont}$, and are centered
about two points along the body, at $s = 0, \frac{L}{2}$. A ground
contact segment extending beyond the head of the body, at $s =
\frac{L}{2}$, wraps-around to continue from the tail end, at $s =
-\frac{L}{2}$. 

Time-coordination between the gait shape $\gSpace(s,  t)$ in \eqref{gait_shape}
and 
body-ground contact $\mathcal{S}_{\rm cont}(t)$ in \eqref{tip_contact}
results in a robot motion pattern that appears like `rotational stepping'. 
The robot begins with a straight-body at the start of the gait. 
Over $t \in [0, \frac{T}{2})$ it picks up interior segments of the body
as $\gSpace(s, t)$ evolves following a standing wave configuration with
peak amplitude, $\bar{A}$. Over $t \in [\frac{T}{2}, T)$ the entire body
achieves ground contact as the gait shape recedes back to a
straight-line configuration. This motion pattern produces a net change
in orientation over a single gait cycle, with little translational
displacement.  We presume the Turn-in-Place gait evolves in a
quasi-static manner; contact segments, $\mathcal{S}_{\rm cont}(t)$, provide mechanical stability for the robot throughout
the gait cycle.



==> 14212207533/arxiv_submission/dynamics.tex <==
The shape-centric modeling approach for deriving the locomotive dynamics
of prescribed gaits \cite{ChVe_RAS[2020]} applies to the Turn-in-Place
gait. This section these dynamics to said gait. 

The configuration space, for snake-like robots entails a 
a shape component, $r \in M$, and a group component, $g \in SE(2)$. 
The shape, $r$, is assumed to be fully controlled such that its dynamics
are prescribed by $u$. Modeling emphasis is on the group dynamics of the
robot, as influenced by its shape kinematics and external forces.  
Second-order dynamical equations that focus on the Lie group structure
are 
\begin{equation} \eqlabel{mech_sys_eoms}
  \myvector{ \dot r \\ \dot g \\ \dot p}
  = 
  \myvector{u \\ 
            g \of{\body \Omega - \loc\Pconn(r, u)} \\ 
            \dual\ad_{\of{\body \Omega - \loc\Pconn(r, u)}} p
              + \body{\mathcal{F}}(r,p,u)},
\end{equation}
where $u$ is the shape space control signal. 
The local principle connection $\loc\Pconn(r, u)$ splits the body
velocity, $\xi^b = \inverse{g} \dot g$, into horizontal and vertical
components with $\body \Omega$ denoting the vertical body velocity
component and $p = \lock\li(r) \body \Omega$ the vertical momentum. 
The horizontal body velocity $\loc\Pconn(r, u)$ describes free-space
motion of the body due to shape kinematics.  Vertical components are
driven by external forcing.  The net external wrench,
$\body{\mathcal{F}}$, acts on the body frame and models this external
forcing.  The dual adjoint operation captures Coriolis effects in the
system.

Additional modeling elements must be computed to specialize the generalized dynamics to the Turn-in-Place gait. 
First, the locked inertia tensor associated with the gait is computed as, 
\begin{equation} \eqlabel{gait_locked_inertia}
  \lock{\li}(\gSpace(s)) 
  = \Int[-\frac{L}{2}]{\frac{L}{2}}
        {\partKEM{\ident}{\JJ (s)}{-\gSpace^T(s) \JJ}{\gSpace^T(s) \gSpace(s)}}{s},
\end{equation}
and describes the inertia associated with instantaneous gait shapes,
$\gSpace(s, t)$. Another term denotes dynamic coupling between the robot
shape and group components,
\begin{equation} \eqlabel{gait_princ_conn}
  \KECsym(\gSpace(s), \dot \gSpace(s)) 
    =  \Int[-\frac{L}{2}]{\frac{L}{2}}{\partKEC{R(s)}{-\gSpace^T(s) \JJ R(s)} \dot \gSpace(s)}{s} \!\!\!.
\end{equation} 
$R(s) \in SO(2)$ is the orientation of a local frame $g_{\rm shape}(s)$,
placed at $\gSpace(s)$ with its $x$-axis tangent to the curve, and
\begin{equation} \nonumber
\JJ = \left[ 
 \begin{array}{cc}
 0 & -1 \\
 1 & 0
 \end{array}
 \right ].
\end{equation}

The local connection form $- \loc\Pconn(\gSpace(s), \dot \gSpace(s))$ is computed from these terms and describes free-space motion of the robot body frame due to internal shape changes,
\begin{equation} \eqlabel{conn_form}
\loc\Pconn(\gSpace(s), \dot \gSpace(s)) = -\inverse{\of{\lock{\li}(\gSpace(s))}} \KECsym(\gSpace(s),\dot \gSpace(s)).
\end{equation}
The total body velocity is, $\body \xi = \body \Omega - \loc\Pconn(\gSpace(s), \dot \gSpace(s))$.

\begin{figure*}[t]
\vspace{0.5mm}
\centering
  \begin{subfigure}{0.71\columnwidth}
	\centering
%	\includegraphics[width=\columnwidth]{placeholder.jpg}
  \resizebox{1.0\columnwidth}{!}{\input{tip_stepping_matlab_orient.tex}}
	\caption{Shape-centric Model}
	\label{tip_traj_fan_matlab}
	\end{subfigure}
%	\hfill
  \hspace{-3.2mm}
  \begin{subfigure}{0.685\columnwidth}
	\centering
%	\includegraphics[width=\columnwidth]{placeholder.jpg}
  \resizebox{1.0\columnwidth}{!}{\input{tip_stepping_gz_orient.tex}}
	\caption{Gazebo}
	\label{tip_traj_fan_gz}
	\end{subfigure}
%	\hfill
  \hspace{-3.2mm}
  \begin{subfigure}{0.685\columnwidth}
	\centering
%	\includegraphics[width=\columnwidth]{placeholder.jpg}
  \resizebox{1.0\columnwidth}{!}{\input{tip_stepping_exp_orient.tex}}
	\caption{Physical Experiment}
	\label{tip_traj_fan_exp}
	\end{subfigure}
	\caption{Trajectories of the robot are tracked over a series of Turn-in-Place experiments, where the gait's peak amplitude $\bar{A}$ is varied from $-120$ mm (red) to $120$ mm (green). In each experiment, $10$ gait cycles are run. A set of experiments is run in each of: \textbf{(a)} \textit{shape-centric model} numerical integration, \textbf{(b)} \textit{Gazebo simulation} and \textbf{(c)} \textit{physical experiment}. In the latter two, the Turn-in-Place gait is implemented on a $12$-link arculated snake-like robot.} 
	\label{tip_traj_fan_compare}
\end{figure*}
\begin{figure*}[t]
\centering
  \begin{subfigure}{0.69\columnwidth}
	\centering
  \resizebox{1.0\columnwidth}{!}{\input{tip_ctrl2action_map_matlab.tex}}
  	\caption{Shape-centric Model}
	\label{cntrl2act_tip_matlab}
	\end{subfigure}
%	\hfill
  \hspace{-3.2mm}
  \begin{subfigure}{0.69\columnwidth}
	\centering
  \resizebox{1.0\columnwidth}{!}{\input{tip_ctrl2action_map_gz.tex}} 
  	\caption{Gazebo}
	\label{cntrl2act_tip_gz}
	\end{subfigure}
%	\hfill
  \hspace{-3.2mm}
  \begin{subfigure}{0.69\columnwidth}
	\centering
  \resizebox{1.0\columnwidth}{!}{\input{tip_ctrl2action_map_exp.tex}} 
  	\caption{Physical Experiment}
	\label{cntrl2act_tip_exp}
	\end{subfigure}
	\caption{Time-averaged, steady-behavior body velocities, $\bar{\bm{\xi}}^b$, computed over $20$ gait cycles of the Turn-in-Place gait, for a range of $\bar{A}$. This may alternatively be interpreted as a control-to-action map, denoted $\bm{\Phi}^{\rm TiP}(\bar{A})$. Red markers denote sampled values; blue plots represent linear fits. A set of experiments is run in each of: \textbf{(a)} \textit{shape-centric model} numerical integration, \textbf{(b)} \textit{Gazebo simulation} and \textbf{(c)} \textit{physical experiment}. The latter two, entail a $12$-link arculated snake-like robot.} 
	\label{cntrl2act_tip_compare}
\end{figure*}

\subsection{Body-Environment Forcing}
We apply viscous friction to model robot-environment interactions. Coefficients $\mu_{\rm b}$, $\mu_{\rm f}$ and $\mu_{\rm n}$ denote resistance to posteriorly-, anteriorly- and laterally-directed motion of the body relative to the ground.
At each point of body-ground contact, $s$, frictional forcing is
computed in the local frame $\gshape(s)$ located at $\gSpace(s)$:
\begin{equation} \eqlabel{local_friction_force}
f(s) = \left[ \begin{array}{c} 
-(\mu_{\rm b} H(-v_x(s)) + \mu_{\rm f} H(v_x(s)))v_x(s) \\
-\mu_{\rm n} v_y(s) \end{array} \right].
\end{equation}
$v(s) = \left[ v_x(s) \hspace{3mm} v_y(s) \right]^T$
describes velocity of the body at $\gSpace(s)$ in the local frame $\gshape(s)$.
$H(\phi)$ denotes the Heaviside step function,
\begin{equation}
  H(\phi) = \small \begin{cases}
              0 & \phi \leq 0 \\
              1 & \phi > 0
            \end{cases}.
\end{equation}
Velocity at each point of body-ground contact, $s \in \mathcal{S}_{\rm cont}$, expressed in the local frame at $\gshape(s)$, has contributions from body frame motion and the local shape derivative, 
\begin{equation} \eqlabel{contrib_shape_vel}
\begin{split}
  v(s) = {\rm linear}\of{\inverse\Ad_{\gshape(s)} \body\xi} + R^{-1}_{\rm shape}(s) \dot{r}(s).
\end{split}
\end{equation}

Integration of external forcing acting along the body, after rigid translation to the body frame, 
produces the net wrench acting at the body frame,
\begin{equation} \eqlabel{body_wrench_form}
\begin{split}
  \body{\mathcal{F}} & 
    = \Int[\mathcal{S}_{\rm cont}]{}
        {\of{\inverse\Ad_{\gshape(s)}}^T \cdot f(s)}{s}.
\end{split}
\end{equation}

\subsection{Model Validation}

The terms \eqref{gait_locked_inertia}, \eqref{conn_form} and
\eqref{body_wrench_form} based on the Turn-in-Place gait shape equations
\eqref{gait_shape} and \eqref{tip_contact}, lead to a set of
integro-differential equations for \eqref{mech_sys_eoms}. 
We validate the equations using the Gazebo simulator and physical
experiments, where the Turn-in-Place gait is implemented on a $12$-link
articulated snake-like robot. 
Sweeping over a range of peak amplitude values, $\bar{A}$, and tracking the
resulting body frame trajectories produces the plots in
Figs.~\ref{tip_traj_fan_matlab}, \ref{tip_traj_fan_gz},
and \ref{tip_traj_fan_exp} for the numerical integration of
\eqref{mech_sys_eoms}, Gazebo simulation, and robot implementation.
Trajectories produced across the three experiment classes
illustrate quantitatively consistent orientation trajectories and small
net translation.  Time-averaged body velocity measurements are plotted
in Figure \ref{cntrl2act_tip_compare}; angular velocity trends linearly
and identically across the experiment classes. 

Discrepancies occur in the translational outcomes of Figs.
\ref{tip_traj_fan_compare}a-c (bottom $2$ plots) and Figs.
\ref{cntrl2act_tip_compare}a-c (top $2$ plots). Several circumstances
lead to the differences. 
The articulated snake-like robot used in Gazebo simulation and physical
experiment will have slightly different governing equations relative to
the continuous body model employed in the shape-centric framework
\cite{ChVe_RAS[2020]}.
Additionally, the physical robot is designed to produce anisotropic
friction between its body and ground \cite{ChVe_Robotica[2019]}, which
results in the larger net translational displacements of Figs.~%
\ref{tip_traj_fan_exp} and \ref{cntrl2act_tip_exp}.  Regardless, net
translational displacement in all experiments remains small, less than
half a body length over $10$ gait cycles ($\bar{L} = 800$ mm).

\subsection{Control-to-Action Behavior}
At steady-behavior, the time-averaged body velocity of an undulatory
gait is a useful characterization of its locomotive behavior. 
The time-averaged body velocity was measured for the Turn-in-Place gait
in all $3$ sets of experiments. After reaching a steady-state behavior,
the three body velocity components were time-averaged over several gait
cycles; see results depicted in Fig.~\ref{cntrl2act_tip_compare}.
Time-averaged body velocities were measured (red markers) for a range of
$\bar{A}$ values, with the polynomial fit curve superimposed (blue).

The curve fit provides a closed-form, approximate representation of the
time-averaged body velocity, as a function of $\bar{A}$. Its defines a
control-to-action map denoted as $\bm{\Phi}^{\rm TiP}(\bar{A}):
\mathbb{R} \to \mathbb{R}^3$.  It maps the gait's input parameter,
$\bar{A}$, to the resulting time-averaged body velocity twist $\xi^b$,
and captures the gait's locomotive behavior as a kinematic motion model.
This reduced motion model supports trajectory planning and tracking for
snake-like robots (see \S \secref{plan_track}).

The Gazebo simulator regressed control-to-action map is
\begin{equation} \eqlabel{cntrl2action_TiP}
\bm{\Phi}^{\rm TiP}(\bar{A}) = \mymatrix{5.3 \text{ mm/s} \\ 0 \text{ mm/s}\\ -0.0382 \cdot \bar{A} + 0.0352\text{ deg/s}}.
\end{equation}
It entails a small positive forward bias, trivial lateral velocity, and
linearly varying angular velocity (w.r.t.~$\bar{A}$). 
The range $\bar{A} \in \left[ -120, 120 \right]$ mm reflects saturation
limits based on the shapes achievable by the 12-link articulated
snake-like robot.

\subsection{Shape-centric Modeling}
The Turn-in-Place gait dynamics were derived using a shape-centric
modeling approach \cite{ChVe_RAS[2020]}.  The shape-centric modeling
framework presents a unified approach to
\begin{enumerate}
 \item define continuous-body shape kinematics, and
 \item derive associated locomotive dynamics,
\end{enumerate}
for gaits employed by limbless, elongated-body mobile robots. 
The modeling framework has been used to model a variety of gaits including 
a caterpillar-like rectilinear gait, lateral undulation, and sidewinding 
\cite{ChVe_RAS[2020], ChSeVe_CDC[2016b]}. Here, we demonstrate this
modeling approach additionally describes the locomotive behavior of a
very different gait: a turn-in-place motion primitive.  Characterization
of the gaits' steady-state locomotive behaviors leads to uniformly
structured control-to-action maps. The reduced-order motion
models simplify these gaits' dynamics to differential drive-like
kinematic motion models useful for planning and control.


==> 14212207536/arxiv_submission/tip_ctrl2action_map_gz.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=7.250in,
height=1.400in,
at={(1.213in,3.800in)},
scale only axis,
xmin=-120,
xmax=120,
xtick={-120, -80, -40, 0, 40, 80, 120},
xticklabels={},
ymin=-10,
ymax=40,
ylabel style={font=\color{white}},
ylabel={\Huge $\bar{\xi}^b_x$ (mm/s)},
axis background/.style={fill=white},
every tick label/.append style={font=\LARGE},
xticklabel style={yshift=-4pt},
yticklabel style={xshift=-3pt},
xtick pos=left,
ytick pos=left,
%axis x line*=bottom,
%axis y line*=left,
%xmajorgrids,
%ymajorgrids
]
\addplot [color=blue, forget plot, line width=2.0pt]
  table[row sep=crcr]{%
-150	5.26743247643731\\
-146.969696969697	5.26743247643731\\
-143.939393939394	5.26743247643731\\
-140.909090909091	5.26743247643731\\
-137.878787878788	5.26743247643731\\
-134.848484848485	5.26743247643731\\
-131.818181818182	5.26743247643731\\
-128.787878787879	5.26743247643731\\
-125.757575757576	5.26743247643731\\
-122.727272727273	5.26743247643731\\
-119.69696969697	5.26743247643731\\
-116.666666666667	5.26743247643731\\
-113.636363636364	5.26743247643731\\
-110.606060606061	5.26743247643731\\
-107.575757575758	5.26743247643731\\
-104.545454545455	5.26743247643731\\
-101.515151515152	5.26743247643731\\
-98.4848484848485	5.26743247643731\\
-95.4545454545455	5.26743247643731\\
-92.4242424242424	5.26743247643731\\
-89.3939393939394	5.26743247643731\\
-86.3636363636364	5.26743247643731\\
-83.3333333333333	5.26743247643731\\
-80.3030303030303	5.26743247643731\\
-77.2727272727273	5.26743247643731\\
-74.2424242424242	5.26743247643731\\
-71.2121212121212	5.26743247643731\\
-68.1818181818182	5.26743247643731\\
-65.1515151515152	5.26743247643731\\
-62.1212121212121	5.26743247643731\\
-59.0909090909091	5.26743247643731\\
-56.0606060606061	5.26743247643731\\
-53.030303030303	5.26743247643731\\
-50	5.26743247643731\\
-46.969696969697	5.26743247643731\\
-43.9393939393939	5.26743247643731\\
-40.9090909090909	5.26743247643731\\
-37.8787878787879	5.26743247643731\\
-34.8484848484849	5.26743247643731\\
-31.8181818181818	5.26743247643731\\
-28.7878787878788	5.26743247643731\\
-25.7575757575758	5.26743247643731\\
-22.7272727272727	5.26743247643731\\
-19.6969696969697	5.26743247643731\\
-16.6666666666667	5.26743247643731\\
-13.6363636363636	5.26743247643731\\
-10.6060606060606	5.26743247643731\\
-7.57575757575758	5.26743247643731\\
-4.54545454545455	5.26743247643731\\
-1.51515151515152	5.26743247643731\\
1.51515151515152	5.26743247643731\\
4.54545454545455	5.26743247643731\\
7.57575757575758	5.26743247643731\\
10.6060606060606	5.26743247643731\\
13.6363636363636	5.26743247643731\\
16.6666666666667	5.26743247643731\\
19.6969696969697	5.26743247643731\\
22.7272727272727	5.26743247643731\\
25.7575757575758	5.26743247643731\\
28.7878787878788	5.26743247643731\\
31.8181818181818	5.26743247643731\\
34.8484848484849	5.26743247643731\\
37.8787878787879	5.26743247643731\\
40.9090909090909	5.26743247643731\\
43.9393939393939	5.26743247643731\\
46.969696969697	5.26743247643731\\
50	5.26743247643731\\
53.030303030303	5.26743247643731\\
56.0606060606061	5.26743247643731\\
59.0909090909091	5.26743247643731\\
62.1212121212121	5.26743247643731\\
65.1515151515152	5.26743247643731\\
68.1818181818182	5.26743247643731\\
71.2121212121212	5.26743247643731\\
74.2424242424242	5.26743247643731\\
77.2727272727273	5.26743247643731\\
80.3030303030303	5.26743247643731\\
83.3333333333333	5.26743247643731\\
86.3636363636364	5.26743247643731\\
89.3939393939394	5.26743247643731\\
92.4242424242424	5.26743247643731\\
95.4545454545455	5.26743247643731\\
98.4848484848485	5.26743247643731\\
101.515151515152	5.26743247643731\\
104.545454545455	5.26743247643731\\
107.575757575758	5.26743247643731\\
110.606060606061	5.26743247643731\\
113.636363636364	5.26743247643731\\
116.666666666667	5.26743247643731\\
119.69696969697	5.26743247643731\\
122.727272727273	5.26743247643731\\
125.757575757576	5.26743247643731\\
128.787878787879	5.26743247643731\\
131.818181818182	5.26743247643731\\
134.848484848485	5.26743247643731\\
137.878787878788	5.26743247643731\\
140.909090909091	5.26743247643731\\
143.939393939394	5.26743247643731\\
146.969696969697	5.26743247643731\\
150	5.26743247643731\\
};
\addplot[only marks, mark=*, mark options={}, mark size=3.0000pt, draw=red, fill=red, forget plot] table[row sep=crcr]{%
x	y\\
-150	11.621087499172\\
-140	10.4172352319195\\
-130	14.1794367325048\\
-120	9.55511919666916\\
-110	6.93782671286851\\
-100	6.06431776862888\\
-90	4.78281117111568\\
-80	3.0634407166068\\
-70	3.54273352778262\\
-60	3.69330628815568\\
-50	2.65373354216494\\
-40	1.97308909758348\\
-30	-0.242161042187058\\
-20	2.22777603316473\\
-10	0.948590166194329\\
0	2.07382939998176\\
10	0.694217646819007\\
20	1.80079787337415\\
30	2.31119014920383\\
40	2.80440611031981\\
50	1.93857925244189\\
60	2.15770536463207\\
70	3.41277178119745\\
80	2.83239215720634\\
90	4.64697257785144\\
100	5.90533348104184\\
110	7.33786084681507\\
120	9.03512014860243\\
130	12.5843298840279\\
140	10.9468923919705\\
150	11.389665061727\\
};
\end{axis}

\begin{axis}[%
width=7.250in,
height=1.400in,
at={(1.213in,2.000in)},
scale only axis,
xmin=-120,
xmax=120,
xtick={-120, -80, -40, 0, 40, 80, 120},
xticklabels={},
ymin=-10,
ymax=10,
ytick={-10, 0, 10},
ylabel style={font=\color{white}},
ylabel={\Huge $\bar{\xi}^b_y$ (mm/s)},
axis background/.style={fill=white},
every tick label/.append style={font=\LARGE},
xticklabel style={yshift=-4pt},
yticklabel style={xshift=-3pt},
xtick pos=left,
ytick pos=left,
%axis x line*=bottom,
%axis y line*=left,
%xmajorgrids,
%ymajorgrids
]
\addplot [color=blue, forget plot, line width=2.0pt]
  table[row sep=crcr]{%
-150	0.318820530900887\\
-146.969696969697	0.318820530900887\\
-143.939393939394	0.318820530900887\\
-140.909090909091	0.318820530900887\\
-137.878787878788	0.318820530900887\\
-134.848484848485	0.318820530900887\\
-131.818181818182	0.318820530900887\\
-128.787878787879	0.318820530900887\\
-125.757575757576	0.318820530900887\\
-122.727272727273	0.318820530900887\\
-119.69696969697	0.318820530900887\\
-116.666666666667	0.318820530900887\\
-113.636363636364	0.318820530900887\\
-110.606060606061	0.318820530900887\\
-107.575757575758	0.318820530900887\\
-104.545454545455	0.318820530900887\\
-101.515151515152	0.318820530900887\\
-98.4848484848485	0.318820530900887\\
-95.4545454545455	0.318820530900887\\
-92.4242424242424	0.318820530900887\\
-89.3939393939394	0.318820530900887\\
-86.3636363636364	0.318820530900887\\
-83.3333333333333	0.318820530900887\\
-80.3030303030303	0.318820530900887\\
-77.2727272727273	0.318820530900887\\
-74.2424242424242	0.318820530900887\\
-71.2121212121212	0.318820530900887\\
-68.1818181818182	0.318820530900887\\
-65.1515151515152	0.318820530900887\\
-62.1212121212121	0.318820530900887\\
-59.0909090909091	0.318820530900887\\
-56.0606060606061	0.318820530900887\\
-53.030303030303	0.318820530900887\\
-50	0.318820530900887\\
-46.969696969697	0.318820530900887\\
-43.9393939393939	0.318820530900887\\
-40.9090909090909	0.318820530900887\\
-37.8787878787879	0.318820530900887\\
-34.8484848484849	0.318820530900887\\
-31.8181818181818	0.318820530900887\\
-28.7878787878788	0.318820530900887\\
-25.7575757575758	0.318820530900887\\
-22.7272727272727	0.318820530900887\\
-19.6969696969697	0.318820530900887\\
-16.6666666666667	0.318820530900887\\
-13.6363636363636	0.318820530900887\\
-10.6060606060606	0.318820530900887\\
-7.57575757575758	0.318820530900887\\
-4.54545454545455	0.318820530900887\\
-1.51515151515152	0.318820530900887\\
1.51515151515152	0.318820530900887\\
4.54545454545455	0.318820530900887\\
7.57575757575758	0.318820530900887\\
10.6060606060606	0.318820530900887\\
13.6363636363636	0.318820530900887\\
16.6666666666667	0.318820530900887\\
19.6969696969697	0.318820530900887\\
22.7272727272727	0.318820530900887\\
25.7575757575758	0.318820530900887\\
28.7878787878788	0.318820530900887\\
31.8181818181818	0.318820530900887\\
34.8484848484849	0.318820530900887\\
37.8787878787879	0.318820530900887\\
40.9090909090909	0.318820530900887\\
43.9393939393939	0.318820530900887\\
46.969696969697	0.318820530900887\\
50	0.318820530900887\\
53.030303030303	0.318820530900887\\
56.0606060606061	0.318820530900887\\
59.0909090909091	0.318820530900887\\
62.1212121212121	0.318820530900887\\
65.1515151515152	0.318820530900887\\
68.1818181818182	0.318820530900887\\
71.2121212121212	0.318820530900887\\
74.2424242424242	0.318820530900887\\
77.2727272727273	0.318820530900887\\
80.3030303030303	0.318820530900887\\
83.3333333333333	0.318820530900887\\
86.3636363636364	0.318820530900887\\
89.3939393939394	0.318820530900887\\
92.4242424242424	0.318820530900887\\
95.4545454545455	0.318820530900887\\
98.4848484848485	0.318820530900887\\
101.515151515152	0.318820530900887\\
104.545454545455	0.318820530900887\\
107.575757575758	0.318820530900887\\
110.606060606061	0.318820530900887\\
113.636363636364	0.318820530900887\\
116.666666666667	0.318820530900887\\
119.69696969697	0.318820530900887\\
122.727272727273	0.318820530900887\\
125.757575757576	0.318820530900887\\
128.787878787879	0.318820530900887\\
131.818181818182	0.318820530900887\\
134.848484848485	0.318820530900887\\
137.878787878788	0.318820530900887\\
140.909090909091	0.318820530900887\\
143.939393939394	0.318820530900887\\
146.969696969697	0.318820530900887\\
150	0.318820530900887\\
};
\addplot[only marks, mark=*, mark options={}, mark size=3.0000pt, draw=red, fill=red, forget plot] table[row sep=crcr]{%
x	y\\
-150	-3.27723659765695\\
-140	-1.43142305936857\\
-130	-1.61931135917822\\
-120	-1.22697824575007\\
-110	-0.441250563774035\\
-100	-0.131658897338902\\
-90	-1.02572339983071\\
-80	-1.37874944882095\\
-70	-1.84207246866203\\
-60	-0.00896955014084487\\
-50	-0.495269663890398\\
-40	0.426755838085617\\
-30	4.07500195881849\\
-20	0.361592589396122\\
-10	0.0828496643713898\\
0	-0.0197872148095936\\
10	-0.166269761100509\\
20	-0.44822866314398\\
30	-0.729225463726852\\
40	-0.750713406655434\\
50	3.53868882601979\\
60	1.0834859207725\\
70	0.525928079230544\\
80	1.0004799608475\\
90	0.781692419150584\\
100	2.09462405365523\\
110	2.83943983646031\\
120	1.27146429726923\\
130	2.19361241155095\\
140	1.32973491098185\\
150	3.27095345516542\\
};
\end{axis}

\begin{axis}[%
width=7.250in,
height=1.400in,
at={(1.213in,0.200in)},
scale only axis,
xmin=-120,
xmax=120,
xtick={-120, -80, -40, 0, 40, 80, 120},
xlabel style={font=\color{white!15!black}},
xlabel={\Huge $\bar{A}$ (mm)},
ymin=-10,
ymax=10,
ytick={-10, 0, 10},
ylabel style={font=\color{white}},
ylabel={\Huge $\bar{\xi}^b_\omega$ (deg/s)},
axis background/.style={fill=white},
every tick label/.append style={font=\LARGE},
xticklabel style={yshift=-4pt},
yticklabel style={xshift=-3pt},
xtick pos=left,
ytick pos=left,
%axis x line*=bottom,
%axis y line*=left,
%xmajorgrids,
%ymajorgrids
]
\addplot [color=blue, forget plot, line width=2.0pt]
  table[row sep=crcr]{%
-150	-5.76452658050554\\
-146.969696969697	-5.64878311648846\\
-143.939393939394	-5.53303965247138\\
-140.909090909091	-5.41729618845431\\
-137.878787878788	-5.30155272443723\\
-134.848484848485	-5.18580926042016\\
-131.818181818182	-5.07006579640308\\
-128.787878787879	-4.95432233238601\\
-125.757575757576	-4.83857886836893\\
-122.727272727273	-4.72283540435186\\
-119.69696969697	-4.60709194033478\\
-116.666666666667	-4.49134847631771\\
-113.636363636364	-4.37560501230063\\
-110.606060606061	-4.25986154828355\\
-107.575757575758	-4.14411808426648\\
-104.545454545455	-4.0283746202494\\
-101.515151515152	-3.91263115623233\\
-98.4848484848485	-3.79688769221525\\
-95.4545454545455	-3.68114422819818\\
-92.4242424242424	-3.5654007641811\\
-89.3939393939394	-3.44965730016403\\
-86.3636363636364	-3.33391383614695\\
-83.3333333333333	-3.21817037212988\\
-80.3030303030303	-3.1024269081128\\
-77.2727272727273	-2.98668344409572\\
-74.2424242424242	-2.87093998007865\\
-71.2121212121212	-2.75519651606157\\
-68.1818181818182	-2.6394530520445\\
-65.1515151515152	-2.52370958802742\\
-62.1212121212121	-2.40796612401035\\
-59.0909090909091	-2.29222265999327\\
-56.0606060606061	-2.1764791959762\\
-53.030303030303	-2.06073573195912\\
-50	-1.94499226794204\\
-46.969696969697	-1.82924880392497\\
-43.9393939393939	-1.71350533990789\\
-40.9090909090909	-1.59776187589082\\
-37.8787878787879	-1.48201841187374\\
-34.8484848484849	-1.36627494785667\\
-31.8181818181818	-1.25053148383959\\
-28.7878787878788	-1.13478801982252\\
-25.7575757575758	-1.01904455580544\\
-22.7272727272727	-0.903301091788364\\
-19.6969696969697	-0.787557627771289\\
-16.6666666666667	-0.671814163754213\\
-13.6363636363636	-0.556070699737138\\
-10.6060606060606	-0.440327235720062\\
-7.57575757575758	-0.324583771702987\\
-4.54545454545455	-0.208840307685911\\
-1.51515151515152	-0.0930968436688356\\
1.51515151515152	0.02264662034824\\
4.54545454545455	0.138390084365315\\
7.57575757575758	0.254133548382391\\
10.6060606060606	0.369877012399467\\
13.6363636363636	0.485620476416542\\
16.6666666666667	0.601363940433617\\
19.6969696969697	0.717107404450693\\
22.7272727272727	0.832850868467769\\
25.7575757575758	0.948594332484844\\
28.7878787878788	1.06433779650192\\
31.8181818181818	1.180081260519\\
34.8484848484849	1.29582472453607\\
37.8787878787879	1.41156818855315\\
40.9090909090909	1.52731165257022\\
43.9393939393939	1.6430551165873\\
46.969696969697	1.75879858060437\\
50	1.87454204462145\\
53.030303030303	1.99028550863852\\
56.0606060606061	2.1060289726556\\
59.0909090909091	2.22177243667267\\
62.1212121212121	2.33751590068975\\
65.1515151515152	2.45325936470683\\
68.1818181818182	2.5690028287239\\
71.2121212121212	2.68474629274098\\
74.2424242424242	2.80048975675805\\
77.2727272727273	2.91623322077513\\
80.3030303030303	3.0319766847922\\
83.3333333333333	3.14772014880928\\
86.3636363636364	3.26346361282635\\
89.3939393939394	3.37920707684343\\
92.4242424242424	3.49495054086051\\
95.4545454545455	3.61069400487758\\
98.4848484848485	3.72643746889466\\
101.515151515152	3.84218093291173\\
104.545454545455	3.95792439692881\\
107.575757575758	4.07366786094588\\
110.606060606061	4.18941132496296\\
113.636363636364	4.30515478898003\\
116.666666666667	4.42089825299711\\
119.69696969697	4.53664171701419\\
122.727272727273	4.65238518103126\\
125.757575757576	4.76812864504834\\
128.787878787879	4.88387210906541\\
131.818181818182	4.99961557308249\\
134.848484848485	5.11535903709956\\
137.878787878788	5.23110250111664\\
140.909090909091	5.34684596513371\\
143.939393939394	5.46258942915079\\
146.969696969697	5.57833289316787\\
150	5.69407635718494\\
};
\addplot[only marks, mark=*, mark options={}, mark size=3.0000pt, draw=red, fill=red, forget plot] table[row sep=crcr]{%
x	y\\
-150	-6.08726820410098\\
-140	-6.00809916312583\\
-130	-5.33776570591697\\
-120	-4.91844043477713\\
-110	-4.32488657449439\\
-100	-3.45893487970239\\
-90	-3.10104850911447\\
-80	-2.60744678123024\\
-70	-2.17870162157346\\
-60	-1.95749526878577\\
-50	-1.52728544226594\\
-40	-1.31071370758424\\
-30	-0.42289061160679\\
-20	-0.684117377751335\\
-10	-0.279885064328275\\
0	0.0100440677849073\\
10	0.349783758620431\\
20	0.719906549273936\\
30	1.03042196539845\\
40	1.35536225384238\\
50	-0.017662109410552\\
60	1.80950404522279\\
70	2.29837168652319\\
80	2.42592087392276\\
90	3.08705786490138\\
100	3.54999802458578\\
110	4.11697332085564\\
120	4.68437551800623\\
130	5.58942904260026\\
140	5.87920579290081\\
150	6.22430822986059\\
};
\end{axis}
\end{tikzpicture}%


==> 14212207536/arxiv_submission/tip_ctrl2action_map_matlab.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=7.250in,
height=1.400in,
at={(1.213in,3.800in)},
scale only axis,
xmin=-120,
xmax=120,
xtick={-120, -80, -40, 0, 40, 80, 120},
xlabel style={font=\color{white!15!black}},
xticklabels={},
%xlabel={\LARGE $\bar{A}$ (mm)},
ymin=-10,
ymax=40,
ylabel style={font=\color{white!15!black},yshift=15pt},
ylabel={\Huge $\bar{\xi}^b_{x}$ (mm/s)},
axis background/.style={fill=white},
every tick label/.append style={font=\LARGE},
xticklabel style={yshift=-4pt},
yticklabel style={xshift=-3pt},
xtick pos=left,
ytick pos=left,
%axis x line*=bottom,
%axis y line*=left,
%xmajorgrids,
%ymajorgrids
]
\addplot [color=blue, forget plot, line width=2.0pt]
  table[row sep=crcr]{%
-150	0.889695310533561\\
-146.969696969697	0.889695310533561\\
-143.939393939394	0.889695310533561\\
-140.909090909091	0.889695310533561\\
-137.878787878788	0.889695310533561\\
-134.848484848485	0.889695310533561\\
-131.818181818182	0.889695310533561\\
-128.787878787879	0.889695310533561\\
-125.757575757576	0.889695310533561\\
-122.727272727273	0.889695310533561\\
-119.69696969697	0.889695310533561\\
-116.666666666667	0.889695310533561\\
-113.636363636364	0.889695310533561\\
-110.606060606061	0.889695310533561\\
-107.575757575758	0.889695310533561\\
-104.545454545455	0.889695310533561\\
-101.515151515152	0.889695310533561\\
-98.4848484848485	0.889695310533561\\
-95.4545454545455	0.889695310533561\\
-92.4242424242424	0.889695310533561\\
-89.3939393939394	0.889695310533561\\
-86.3636363636364	0.889695310533561\\
-83.3333333333333	0.889695310533561\\
-80.3030303030303	0.889695310533561\\
-77.2727272727273	0.889695310533561\\
-74.2424242424242	0.889695310533561\\
-71.2121212121212	0.889695310533561\\
-68.1818181818182	0.889695310533561\\
-65.1515151515152	0.889695310533561\\
-62.1212121212121	0.889695310533561\\
-59.0909090909091	0.889695310533561\\
-56.0606060606061	0.889695310533561\\
-53.030303030303	0.889695310533561\\
-50	0.889695310533561\\
-46.969696969697	0.889695310533561\\
-43.9393939393939	0.889695310533561\\
-40.9090909090909	0.889695310533561\\
-37.8787878787879	0.889695310533561\\
-34.8484848484849	0.889695310533561\\
-31.8181818181818	0.889695310533561\\
-28.7878787878788	0.889695310533561\\
-25.7575757575758	0.889695310533561\\
-22.7272727272727	0.889695310533561\\
-19.6969696969697	0.889695310533561\\
-16.6666666666667	0.889695310533561\\
-13.6363636363636	0.889695310533561\\
-10.6060606060606	0.889695310533561\\
-7.57575757575758	0.889695310533561\\
-4.54545454545455	0.889695310533561\\
-1.51515151515152	0.889695310533561\\
1.51515151515152	0.889695310533561\\
4.54545454545455	0.889695310533561\\
7.57575757575758	0.889695310533561\\
10.6060606060606	0.889695310533561\\
13.6363636363636	0.889695310533561\\
16.6666666666667	0.889695310533561\\
19.6969696969697	0.889695310533561\\
22.7272727272727	0.889695310533561\\
25.7575757575758	0.889695310533561\\
28.7878787878788	0.889695310533561\\
31.8181818181818	0.889695310533561\\
34.8484848484849	0.889695310533561\\
37.8787878787879	0.889695310533561\\
40.9090909090909	0.889695310533561\\
43.9393939393939	0.889695310533561\\
46.969696969697	0.889695310533561\\
50	0.889695310533561\\
53.030303030303	0.889695310533561\\
56.0606060606061	0.889695310533561\\
59.0909090909091	0.889695310533561\\
62.1212121212121	0.889695310533561\\
65.1515151515152	0.889695310533561\\
68.1818181818182	0.889695310533561\\
71.2121212121212	0.889695310533561\\
74.2424242424242	0.889695310533561\\
77.2727272727273	0.889695310533561\\
80.3030303030303	0.889695310533561\\
83.3333333333333	0.889695310533561\\
86.3636363636364	0.889695310533561\\
89.3939393939394	0.889695310533561\\
92.4242424242424	0.889695310533561\\
95.4545454545455	0.889695310533561\\
98.4848484848485	0.889695310533561\\
101.515151515152	0.889695310533561\\
104.545454545455	0.889695310533561\\
107.575757575758	0.889695310533561\\
110.606060606061	0.889695310533561\\
113.636363636364	0.889695310533561\\
116.666666666667	0.889695310533561\\
119.69696969697	0.889695310533561\\
122.727272727273	0.889695310533561\\
125.757575757576	0.889695310533561\\
128.787878787879	0.889695310533561\\
131.818181818182	0.889695310533561\\
134.848484848485	0.889695310533561\\
137.878787878788	0.889695310533561\\
140.909090909091	0.889695310533561\\
143.939393939394	0.889695310533561\\
146.969696969697	0.889695310533561\\
150	0.889695310533561\\
};
\addplot[only marks, mark=*, mark options={}, mark size=3.0000pt, draw=red, fill=red, forget plot] table[row sep=crcr]{%
x	y\\
-150	2.18887812777504\\
-140	1.96966036586464\\
-130	1.7609338504536\\
-120	1.5639148554553\\
-110	1.37149923124033\\
-100	1.18216327000942\\
-90	0.997215945723879\\
-80	0.819046090018085\\
-70	0.650200104407958\\
-60	0.493707488308252\\
-50	0.35303644594328\\
-40	0.231779079090821\\
-30	0.133073453178114\\
-20	0.0600202944302968\\
-10	0.0151487113711818\\
0	0\\
10	0.0151487113711818\\
20	0.0600202944302968\\
30	0.133073453178114\\
40	0.231779079090821\\
50	0.35303644594328\\
60	0.493707488308252\\
70	0.650200104407958\\
80	0.819046090018085\\
90	0.997215945723879\\
100	1.18216327000942\\
110	1.37149923124033\\
120	1.5639148554553\\
130	1.7609338504536\\
140	1.96966036586464\\
150	2.18887812777504\\
};
\end{axis}

\begin{axis}[%
width=7.250in,
height=1.400in,
at={(1.213in,2.000in)},
scale only axis,
xmin=-120,
xmax=120,
xtick={-120, -80, -40, 0, 40, 80, 120},
xlabel style={font=\color{white!15!black}},
xticklabels={},
%xlabel={\LARGE $\bar{A}$ (mm)},
ymin=-10,
ymax=10,
ytick={-10, 0, 10},
ylabel style={font=\color{white!15!black}},
ylabel={\Huge $\bar{\xi}^b_{y}$ (mm/s)},
axis background/.style={fill=white},
every tick label/.append style={font=\LARGE},
xticklabel style={yshift=-4pt},
yticklabel style={xshift=-3pt},
xtick pos=left,
ytick pos=left,
%axis x line*=bottom,
%axis y line*=left,
%xmajorgrids,
%ymajorgrids
]
\addplot [color=blue, forget plot, line width=2.0pt]
  table[row sep=crcr]{%
-150	1.22297174697324e-17\\
-146.969696969697	1.22297174697324e-17\\
-143.939393939394	1.22297174697324e-17\\
-140.909090909091	1.22297174697324e-17\\
-137.878787878788	1.22297174697324e-17\\
-134.848484848485	1.22297174697324e-17\\
-131.818181818182	1.22297174697324e-17\\
-128.787878787879	1.22297174697324e-17\\
-125.757575757576	1.22297174697324e-17\\
-122.727272727273	1.22297174697324e-17\\
-119.69696969697	1.22297174697324e-17\\
-116.666666666667	1.22297174697324e-17\\
-113.636363636364	1.22297174697324e-17\\
-110.606060606061	1.22297174697324e-17\\
-107.575757575758	1.22297174697324e-17\\
-104.545454545455	1.22297174697324e-17\\
-101.515151515152	1.22297174697324e-17\\
-98.4848484848485	1.22297174697324e-17\\
-95.4545454545455	1.22297174697324e-17\\
-92.4242424242424	1.22297174697324e-17\\
-89.3939393939394	1.22297174697324e-17\\
-86.3636363636364	1.22297174697324e-17\\
-83.3333333333333	1.22297174697324e-17\\
-80.3030303030303	1.22297174697324e-17\\
-77.2727272727273	1.22297174697324e-17\\
-74.2424242424242	1.22297174697324e-17\\
-71.2121212121212	1.22297174697324e-17\\
-68.1818181818182	1.22297174697324e-17\\
-65.1515151515152	1.22297174697324e-17\\
-62.1212121212121	1.22297174697324e-17\\
-59.0909090909091	1.22297174697324e-17\\
-56.0606060606061	1.22297174697324e-17\\
-53.030303030303	1.22297174697324e-17\\
-50	1.22297174697324e-17\\
-46.969696969697	1.22297174697324e-17\\
-43.9393939393939	1.22297174697324e-17\\
-40.9090909090909	1.22297174697324e-17\\
-37.8787878787879	1.22297174697324e-17\\
-34.8484848484849	1.22297174697324e-17\\
-31.8181818181818	1.22297174697324e-17\\
-28.7878787878788	1.22297174697324e-17\\
-25.7575757575758	1.22297174697324e-17\\
-22.7272727272727	1.22297174697324e-17\\
-19.6969696969697	1.22297174697324e-17\\
-16.6666666666667	1.22297174697324e-17\\
-13.6363636363636	1.22297174697324e-17\\
-10.6060606060606	1.22297174697324e-17\\
-7.57575757575758	1.22297174697324e-17\\
-4.54545454545455	1.22297174697324e-17\\
-1.51515151515152	1.22297174697324e-17\\
1.51515151515152	1.22297174697324e-17\\
4.54545454545455	1.22297174697324e-17\\
7.57575757575758	1.22297174697324e-17\\
10.6060606060606	1.22297174697324e-17\\
13.6363636363636	1.22297174697324e-17\\
16.6666666666667	1.22297174697324e-17\\
19.6969696969697	1.22297174697324e-17\\
22.7272727272727	1.22297174697324e-17\\
25.7575757575758	1.22297174697324e-17\\
28.7878787878788	1.22297174697324e-17\\
31.8181818181818	1.22297174697324e-17\\
34.8484848484849	1.22297174697324e-17\\
37.8787878787879	1.22297174697324e-17\\
40.9090909090909	1.22297174697324e-17\\
43.9393939393939	1.22297174697324e-17\\
46.969696969697	1.22297174697324e-17\\
50	1.22297174697324e-17\\
53.030303030303	1.22297174697324e-17\\
56.0606060606061	1.22297174697324e-17\\
59.0909090909091	1.22297174697324e-17\\
62.1212121212121	1.22297174697324e-17\\
65.1515151515152	1.22297174697324e-17\\
68.1818181818182	1.22297174697324e-17\\
71.2121212121212	1.22297174697324e-17\\
74.2424242424242	1.22297174697324e-17\\
77.2727272727273	1.22297174697324e-17\\
80.3030303030303	1.22297174697324e-17\\
83.3333333333333	1.22297174697324e-17\\
86.3636363636364	1.22297174697324e-17\\
89.3939393939394	1.22297174697324e-17\\
92.4242424242424	1.22297174697324e-17\\
95.4545454545455	1.22297174697324e-17\\
98.4848484848485	1.22297174697324e-17\\
101.515151515152	1.22297174697324e-17\\
104.545454545455	1.22297174697324e-17\\
107.575757575758	1.22297174697324e-17\\
110.606060606061	1.22297174697324e-17\\
113.636363636364	1.22297174697324e-17\\
116.666666666667	1.22297174697324e-17\\
119.69696969697	1.22297174697324e-17\\
122.727272727273	1.22297174697324e-17\\
125.757575757576	1.22297174697324e-17\\
128.787878787879	1.22297174697324e-17\\
131.818181818182	1.22297174697324e-17\\
134.848484848485	1.22297174697324e-17\\
137.878787878788	1.22297174697324e-17\\
140.909090909091	1.22297174697324e-17\\
143.939393939394	1.22297174697324e-17\\
146.969696969697	1.22297174697324e-17\\
150	1.22297174697324e-17\\
};
\addplot[only marks, mark=*, mark options={}, mark size=3.0000pt, draw=red, fill=red, forget plot] table[row sep=crcr]{%
x	y\\
-150	0.669383934579662\\
-140	0.453311666683995\\
-130	0.31360005759163\\
-120	0.220914741575262\\
-110	0.156313433796564\\
-100	0.109918908608146\\
-90	0.0760878425576844\\
-80	0.0513200595994904\\
-70	0.0333218150411926\\
-60	0.0204565308666246\\
-50	0.0116125519018021\\
-40	0.00589798647419753\\
-30	0.00247344006475824\\
-20	0.000726394003855825\\
-10	9.10587888591914e-05\\
0	0\\
10	-9.10587888591914e-05\\
20	-0.000726394003855825\\
30	-0.00247344006475824\\
40	-0.00589798647419753\\
50	-0.0116125519018021\\
60	-0.0204565308666246\\
70	-0.0333218150411926\\
80	-0.0513200595994904\\
90	-0.0760878425576844\\
100	-0.109918908608146\\
110	-0.156313433796564\\
120	-0.220914741575262\\
130	-0.31360005759163\\
140	-0.453311666683995\\
150	-0.669383934579662\\
};
\end{axis}

\begin{axis}[%
width=7.250in,
height=1.400in,
at={(1.213in,0.200in)},
scale only axis,
xmin=-120,
xmax=120,
xtick={-120, -80, -40, 0, 40, 80, 120},
xlabel style={font=\color{white!15!black}},
xlabel={\Huge $\bar{A}$ (mm)},
ymin=-10,
ymax=10,
ytick={-10, 0, 10},
ylabel style={font=\color{white!15!black}},
ylabel={\Huge $\bar{\xi}^b_{\omega}$ (deg/s)},
axis background/.style={fill=white},
every tick label/.append style={font=\LARGE},
xticklabel style={yshift=-4pt},
yticklabel style={xshift=-3pt},
xtick pos=left,
ytick pos=left,
%axis x line*=bottom,
%axis y line*=left,
%xmajorgrids,
%ymajorgrids
]
\addplot [color=blue, forget plot, line width=2.0pt]
  table[row sep=crcr]{%
-150	-7.29592831363267\\
-146.969696969697	-7.14853582244817\\
-143.939393939394	-7.00114333126368\\
-140.909090909091	-6.85375084007918\\
-137.878787878788	-6.70635834889468\\
-134.848484848485	-6.55896585771018\\
-131.818181818182	-6.41157336652568\\
-128.787878787879	-6.26418087534118\\
-125.757575757576	-6.11678838415668\\
-122.727272727273	-5.96939589297219\\
-119.69696969697	-5.82200340178769\\
-116.666666666667	-5.67461091060319\\
-113.636363636364	-5.52721841941869\\
-110.606060606061	-5.37982592823419\\
-107.575757575758	-5.23243343704969\\
-104.545454545455	-5.0850409458652\\
-101.515151515152	-4.9376484546807\\
-98.4848484848485	-4.7902559634962\\
-95.4545454545455	-4.6428634723117\\
-92.4242424242424	-4.4954709811272\\
-89.3939393939394	-4.3480784899427\\
-86.3636363636364	-4.20068599875821\\
-83.3333333333333	-4.05329350757371\\
-80.3030303030303	-3.90590101638921\\
-77.2727272727273	-3.75850852520471\\
-74.2424242424242	-3.61111603402021\\
-71.2121212121212	-3.46372354283571\\
-68.1818181818182	-3.31633105165121\\
-65.1515151515152	-3.16893856046672\\
-62.1212121212121	-3.02154606928222\\
-59.0909090909091	-2.87415357809772\\
-56.0606060606061	-2.72676108691322\\
-53.030303030303	-2.57936859572872\\
-50	-2.43197610454422\\
-46.969696969697	-2.28458361335973\\
-43.9393939393939	-2.13719112217523\\
-40.9090909090909	-1.98979863099073\\
-37.8787878787879	-1.84240613980623\\
-34.8484848484849	-1.69501364862173\\
-31.8181818181818	-1.54762115743723\\
-28.7878787878788	-1.40022866625273\\
-25.7575757575758	-1.25283617506824\\
-22.7272727272727	-1.10544368388374\\
-19.6969696969697	-0.95805119269924\\
-16.6666666666667	-0.810658701514741\\
-13.6363636363636	-0.663266210330243\\
-10.6060606060606	-0.515873719145744\\
-7.57575757575758	-0.368481227961246\\
-4.54545454545455	-0.221088736776748\\
-1.51515151515152	-0.0736962455922492\\
1.51515151515152	0.0736962455922493\\
4.54545454545455	0.221088736776748\\
7.57575757575758	0.368481227961246\\
10.6060606060606	0.515873719145744\\
13.6363636363636	0.663266210330243\\
16.6666666666667	0.810658701514741\\
19.6969696969697	0.95805119269924\\
22.7272727272727	1.10544368388374\\
25.7575757575758	1.25283617506824\\
28.7878787878788	1.40022866625273\\
31.8181818181818	1.54762115743723\\
34.8484848484849	1.69501364862173\\
37.8787878787879	1.84240613980623\\
40.9090909090909	1.98979863099073\\
43.9393939393939	2.13719112217523\\
46.969696969697	2.28458361335973\\
50	2.43197610454422\\
53.030303030303	2.57936859572872\\
56.0606060606061	2.72676108691322\\
59.0909090909091	2.87415357809772\\
62.1212121212121	3.02154606928222\\
65.1515151515152	3.16893856046672\\
68.1818181818182	3.31633105165121\\
71.2121212121212	3.46372354283571\\
74.2424242424242	3.61111603402021\\
77.2727272727273	3.75850852520471\\
80.3030303030303	3.90590101638921\\
83.3333333333333	4.05329350757371\\
86.3636363636364	4.20068599875821\\
89.3939393939394	4.3480784899427\\
92.4242424242424	4.4954709811272\\
95.4545454545455	4.6428634723117\\
98.4848484848485	4.7902559634962\\
101.515151515152	4.9376484546807\\
104.545454545455	5.0850409458652\\
107.575757575758	5.23243343704969\\
110.606060606061	5.37982592823419\\
113.636363636364	5.52721841941869\\
116.666666666667	5.67461091060319\\
119.69696969697	5.82200340178769\\
122.727272727273	5.96939589297219\\
125.757575757576	6.11678838415668\\
128.787878787879	6.26418087534118\\
131.818181818182	6.41157336652568\\
134.848484848485	6.55896585771018\\
137.878787878788	6.70635834889468\\
140.909090909091	6.85375084007918\\
143.939393939394	7.00114333126368\\
146.969696969697	7.14853582244817\\
150	7.29592831363267\\
};
\addplot[only marks, mark=*, mark options={}, mark size=3.0000pt, draw=red, fill=red, forget plot] table[row sep=crcr]{%
x	y\\
-150	-10.1833683421111\\
-140	-8.2490383523723\\
-130	-6.7531835588896\\
-120	-5.59371357179558\\
-110	-4.64220668621876\\
-100	-3.85793769752333\\
-90	-3.20059778869612\\
-80	-2.64328106726483\\
-70	-2.16405065830002\\
-60	-1.75166886804308\\
-50	-1.38899750254796\\
-40	-1.05910587763514\\
-30	-0.765859036701713\\
-20	-0.499770785782492\\
-10	-0.244886053644276\\
0	0\\
10	0.244886053644276\\
20	0.499770785782492\\
30	0.765859036701713\\
40	1.05910587763514\\
50	1.38899750254796\\
60	1.75166886804308\\
70	2.16405065830002\\
80	2.64328106726483\\
90	3.20059778869612\\
100	3.85793769752333\\
110	4.64220668621876\\
120	5.59371357179558\\
130	6.7531835588896\\
140	8.2490383523723\\
150	10.1833683421111\\
};
\end{axis}
\end{tikzpicture}%


==> 14212207537/arxiv_submission/results.tex <==
\begin{figure*}[t]
  \vspace{1.0mm}
	\centering
  \begin{tikzpicture}[inner sep=0pt, outer sep=0pt]
  	\def\firstScenWidth{0.75\columnwidth}
  	\def\secScenWidth{0.9\columnwidth}
  	\def\thirdScenWidth{0.9\columnwidth}
  	\def\secScenHorizPos{0.85\columnwidth}
  	\def\labScenHorizPos{0.925\columnwidth}
  
    % Place scenario 1 "map" view only.
%    \draw (0in,0in) -- ++(0.5\columnwidth,0in) -- ++(0in, 3in) 
%      -- ++(-0.5\columnwidth,0in) -- cycle;
    	\node[anchor=north west,outer sep=0pt,minimum height=3in,minimum width=\firstScenWidth,draw=none] (scen1_map) at (0in,3in) 
    	{\includegraphics[width=\firstScenWidth]{multigait_scen01_pos_traj.pdf}};
    % Place scenario 2 "map" view only.
%    \draw (0.55\columnwidth,1.5in) -- ++(1.45\columnwidth,0in) 
%      -- ++(0in, 1.5in) -- ++(-1.45\columnwidth,0in) -- cycle;
    \node[anchor=north west,outer sep=0pt,minimum height=1.5in,minimum width=\secScenWidth,draw=none] (scen2_map) at ($(\secScenHorizPos,3in)+(0in,0.1in)$)
    	{\includegraphics[width=\secScenWidth]{multigait_scen02_pos_traj.pdf}};
    % Place scenario 3 "map" view only.
%    \draw (0.55\columnwidth,0in) -- ++(1.45\columnwidth,0in) 
%      -- ++(0in, 1.5in) -- ++(-1.45\columnwidth,0in) -- cycle;
    \node[anchor=north west,outer sep=0pt,minimum height=1.5in,minimum width=\thirdScenWidth,draw=none] (scen3_map) at ($(\secScenHorizPos,1.5in)+(0in,0.1in)$)
    	{\includegraphics[width=\thirdScenWidth]{multigait_scen03_pos_traj.pdf}};

    \node[anchor=north west,outer sep=2pt] at (1.8in,2.9in) {Scenario 1};
    \node[anchor=north west,outer sep=2pt] at (\labScenHorizPos,1.95in) {Scenario 2};
    \node[anchor=north west,outer sep=2pt] at (\labScenHorizPos,1.5in) {Scenario 3};

    \node[anchor=north] at ($(scen1_map)+(-0.20in,-0.25in)$) {\small start};
    \node[anchor=north] at ($(scen2_map)+(-0.30in,0.20in)$) {\small start};
    \node[anchor=north] at ($(scen3_map)+(-0.55in,0.07in)$) {\small start};
    \node[anchor=north] at ($(scen1_map)+(0.80in,0.27in)$) {\small goal};
    \node[anchor=north] at ($(scen2_map)+(0.85in,-0.15in)$) {\small goal};
    \node[anchor=north] at ($(scen3_map)+(1.17in,0.52in)$) {\small goal};
  \end{tikzpicture}
  \caption{Depiction of environments for the three locomotion scenarios,
    with parametric plots of the multi-gait planned and achieved
    (based on tracking) trajectories. The snake-like robot
    successfully maneuvers to the goal in all
    cases.\label{fig:mult-gait-scen}} 
  \vspace*{-1em}
\end{figure*}

This section pairs the Turn-in-Place gait with a translation-dominant
Rectilinear gait and show that a $12$-link snake-like robot
can plan and track trajectories that neither gait alone is capable of
following.  
%The limited steering capabilities of the Rectilinear gait are compensated for by the rotational capabilities of the Turn-in-Place gait.  
Three locomotion scenarios, depicted in Fig.~\ref{fig:mult-gait-scen},
are successfully completed using these two gaits within the multi-gait
trajectory planning and tracking approach presented in
\S\secref{plan_track}.  Rectilinear motion is used for path segments
that require little steering.  The multi-gait planner switches to
Turn-in-Place motion at ``sharp'' corners and is used at the start of
each trajectory to align the robot body frame with the direction of
travel.

Taken together the scenarios require sufficiently diverse motion
profiles that they can be deemed reflective of most navigation scenarios
with comparable free space vs collision space characteristics.
The narrowest passageways have widths equivalent to the robot body
length ($\bar{L} = 800$ mm).  
Tracking errors arise due to initial transients when momentum
accumulates, transitions when gait parameter values change, and
gait switching. These effects are un-modeled and are not considered
as part of the multi-gait trajectory synthesis process.  Discrete-time,
trajectory tracking control corrects for these errors.  

The control and orientation signals are plotted in Figure \ref{signals}.
Their piecewise nature is a function of the active gait changing as a
function of time, and therefore the applied control for the gait.
Whereas Figure \ref{fig:mult-gait-scen} confirms trajectory tracking,
Figure \ref{signals} confirmed orientation tracking (top left graph for
each scenario). Closed-loop discrete control under the empirically
regressed models successfully tracks the synthesized trajectories to
arrive at the goal point.

%In each figure, the left-top plot illustrates the locomotion scenario as well as planned (blue) and and tracked (green) positional trajectories. Orientation trajectories are depicted below this. The right-top and right-middle plots show Turn-in-Place and Rectilinear control signals, respectively, used to traverse each scenario. Planned and tracked angular velocities are depicted in the right-bottom plot.


\begin{figure*}[t]
  \vspace{0.5mm}
  \begin{center}
  % MAKE FIGURES PROPER ASPECT RATIO AND SCALE THEN REMOVE THE SCALEBOX COMMAND.
  \scalebox{0.95}{
  \begin{tikzpicture}[inner sep=0pt, outer sep=0pt]
  		% south west (angular velocity)
    	\node[draw=none,rectangle,minimum width=\columnwidth,minimum height=0.75in,anchor=south west] (B) at (0in,0in)
    {\includegraphics[width=\columnwidth]{multigait_scen01_w_cntrl.pdf}};
  		% north west (orientation trajectory)
    	\node[draw=none,rectangle,minimum width=\columnwidth,minimum height=0.75in,anchor=south west] (A) at ($(B.north west)+(-1.5mm,0in)$)
    {\includegraphics[width=0.98\columnwidth]{multigait_scen01_orient_traj.pdf}};
  		% south east (RL \kappa control) 
    \node[draw=none,rectangle,minimum width=\columnwidth,minimum
    height=0.75in,anchor=south west,xshift=5pt] (D) at (B.south east)
    {\includegraphics[width=\columnwidth]{multigait_scen01_rl_cntrl.pdf}};
  		% north east (TiP \bar{A} control)
    \node[draw=none,rectangle,minimum width=\columnwidth,minimum
    height=0.75in,anchor=south west,xshift=5pt] (C) at ($(A.south east)+(-0.5mm,0in)$)
    {\includegraphics[width=0.99\columnwidth]{multigait_scen01_tip_cntrl.pdf}};
  \end{tikzpicture}}
  \vspace{-2.0mm}
  \subcaption{Scenario 1 signals}
  \vspace{3.0mm}
%\end{figure*}
%\begin{figure*}[t]
  \centering
  % MAKE FIGURES PROPER ASPECT RATIO AND SCALE THEN REMOVE THE SCALEBOX COMMAND.
  \scalebox{0.95}{
  \begin{tikzpicture}[inner sep=0pt, outer sep=0pt]
  		% south west (angular velocity)
    \node[draw=none,rectangle,minimum width=\columnwidth,minimum height=0.75in,anchor=south west] (B) at (0in,0in)
    {\includegraphics[width=0.99\columnwidth]{multigait_scen02_w_cntrl.pdf}};
  		% north west (orientation trajectory)
    	\node[draw=none,rectangle,minimum width=\columnwidth,minimum height=0.75in,anchor=south west] (A) at ($(B.north west)+(+0mm,0in)$)
    {\includegraphics[width=\columnwidth]{multigait_scen02_orient_traj.pdf}};    
  		% south east (RL \kappa control)
    \node[draw=none,rectangle,minimum width=\columnwidth,minimum
    height=0.75in,anchor=south west,xshift=5pt] (D) at (B.south east)
    {\includegraphics[width=0.98\columnwidth]{multigait_scen02_rl_cntrl.pdf}};
  		% north east (TiP \bar{A} control)
    \node[draw=none,rectangle,minimum width=\columnwidth,minimum
    height=0.75in,anchor=south west,xshift=5pt] (C) at ($(A.south east)+(-1.0mm,0in)$)
    {\includegraphics[width=\columnwidth]{multigait_scen02_tip_cntrl.pdf}};
  \end{tikzpicture}}
  \vspace{-2.0mm}
  \subcaption{Scenario 2 signals}
  \vspace{3.0mm}
%\end{figure*}
%\begin{figure*}[t]
  \centering
  % MAKE FIGURES PROPER ASPECT RATIO AND SCALE THEN REMOVE THE SCALEBOX COMMAND.
  \scalebox{0.95}{
  \begin{tikzpicture}[inner sep=0pt, outer sep=0pt]
  		% south west (angular velocity)
    \node[draw=none,rectangle,minimum width=\columnwidth,minimum height=0.75in,anchor=south west] (B) at (0in,0in)
    {\includegraphics[width=\columnwidth]{multigait_scen03_w_cntrl.pdf}};
  		% north west (orientation trajectory)
    	\node[draw=none,rectangle,minimum width=\columnwidth,minimum height=0.75in,anchor=south west] (A) at ($(B.north west)+(-1.5mm,0in)$)
    {\includegraphics[width=0.98\columnwidth]{multigait_scen03_orient_traj.pdf}};
  		% south east (RL \kappa control)
    \node[draw=none,rectangle,minimum width=\columnwidth,minimum
    height=0.75in,anchor=south west,xshift=5pt] (D) at (B.south east)
    {\includegraphics[width=\columnwidth]{multigait_scen03_rl_cntrl.pdf}};
  		% north east (TiP \bar{A} control)
    \node[draw=none,rectangle,minimum width=\columnwidth,minimum
    height=0.75in,anchor=south west,xshift=5pt] (C) at ($(A.south east)+(-0.5mm,0in)$)
    {\includegraphics[width=0.99\columnwidth]{multigait_scen03_tip_cntrl.pdf}};
  \end{tikzpicture}}
  \vspace{-2.0mm}
  \subcaption{Scenario 3 signals.}
  \end{center}
  \caption{Time-varying signals describing Scenarios 1-3 in Figure
  \ref{fig:mult-gait-scen}: \textbf{(top-left)} orientation, $\theta(t)$
  \textbf{(bottom-left)} angular velocity, $\xi^b_{\omega}(t)$
  \textbf{(top-right)} Rectilinear curvature, $\kappa(t)$
  \textbf{(bottom-right)} Turn-in-Place peak amplitude, $\bar{A}(t)$.
  \label{signals}}
  %\vspace*{-2em}
  \vspace{-10.0mm}
\end{figure*}





==> 14212207537/arxiv_submission/tip_ctrl2action_map_exp.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=7.250in,
height=1.400in,
at={(1.213in,3.800in)},
scale only axis,
xmin=-120,
xmax=120,
xtick={-120, -80, -40, 0, 40, 80, 120},
xticklabels={},
ymin=-10,
ymax=40,
ylabel style={font=\color{white}},
ylabel={\Huge $\bar{\xi}^b_x$ (mm/s)},
axis background/.style={fill=white},
every tick label/.append style={font=\LARGE},
xticklabel style={yshift=-4pt},
yticklabel style={xshift=-3pt},
xtick pos=left,
ytick pos=left,
%axis x line*=bottom,
%axis y line*=left,
%xmajorgrids,
%ymajorgrids
]
\addplot [color=blue, forget plot, line width=2.0pt]
  table[row sep=crcr]{%
-120	5.76037886797324\\
-117.575757575758	5.76037886797324\\
-115.151515151515	5.76037886797324\\
-112.727272727273	5.76037886797324\\
-110.30303030303	5.76037886797324\\
-107.878787878788	5.76037886797324\\
-105.454545454545	5.76037886797324\\
-103.030303030303	5.76037886797324\\
-100.606060606061	5.76037886797324\\
-98.1818181818182	5.76037886797324\\
-95.7575757575758	5.76037886797324\\
-93.3333333333333	5.76037886797324\\
-90.9090909090909	5.76037886797324\\
-88.4848484848485	5.76037886797324\\
-86.0606060606061	5.76037886797324\\
-83.6363636363636	5.76037886797324\\
-81.2121212121212	5.76037886797324\\
-78.7878787878788	5.76037886797324\\
-76.3636363636364	5.76037886797324\\
-73.9393939393939	5.76037886797324\\
-71.5151515151515	5.76037886797324\\
-69.0909090909091	5.76037886797324\\
-66.6666666666667	5.76037886797324\\
-64.2424242424242	5.76037886797324\\
-61.8181818181818	5.76037886797324\\
-59.3939393939394	5.76037886797324\\
-56.969696969697	5.76037886797324\\
-54.5454545454545	5.76037886797324\\
-52.1212121212121	5.76037886797324\\
-49.6969696969697	5.76037886797324\\
-47.2727272727273	5.76037886797324\\
-44.8484848484849	5.76037886797324\\
-42.4242424242424	5.76037886797324\\
-40	5.76037886797324\\
-37.5757575757576	5.76037886797324\\
-35.1515151515151	5.76037886797324\\
-32.7272727272727	5.76037886797324\\
-30.3030303030303	5.76037886797324\\
-27.8787878787879	5.76037886797324\\
-25.4545454545455	5.76037886797324\\
-23.030303030303	5.76037886797324\\
-20.6060606060606	5.76037886797324\\
-18.1818181818182	5.76037886797324\\
-15.7575757575758	5.76037886797324\\
-13.3333333333333	5.76037886797324\\
-10.9090909090909	5.76037886797324\\
-8.48484848484848	5.76037886797324\\
-6.06060606060606	5.76037886797324\\
-3.63636363636364	5.76037886797324\\
-1.21212121212121	5.76037886797324\\
1.21212121212121	5.76037886797324\\
3.63636363636364	5.76037886797324\\
6.06060606060606	5.76037886797324\\
8.48484848484848	5.76037886797324\\
10.9090909090909	5.76037886797324\\
13.3333333333333	5.76037886797324\\
15.7575757575758	5.76037886797324\\
18.1818181818182	5.76037886797324\\
20.6060606060606	5.76037886797324\\
23.030303030303	5.76037886797324\\
25.4545454545455	5.76037886797324\\
27.8787878787879	5.76037886797324\\
30.3030303030303	5.76037886797324\\
32.7272727272727	5.76037886797324\\
35.1515151515151	5.76037886797324\\
37.5757575757576	5.76037886797324\\
40	5.76037886797324\\
42.4242424242424	5.76037886797324\\
44.8484848484849	5.76037886797324\\
47.2727272727273	5.76037886797324\\
49.6969696969697	5.76037886797324\\
52.1212121212121	5.76037886797324\\
54.5454545454545	5.76037886797324\\
56.969696969697	5.76037886797324\\
59.3939393939394	5.76037886797324\\
61.8181818181818	5.76037886797324\\
64.2424242424242	5.76037886797324\\
66.6666666666667	5.76037886797324\\
69.0909090909091	5.76037886797324\\
71.5151515151515	5.76037886797324\\
73.9393939393939	5.76037886797324\\
76.3636363636364	5.76037886797324\\
78.7878787878788	5.76037886797324\\
81.2121212121212	5.76037886797324\\
83.6363636363636	5.76037886797324\\
86.0606060606061	5.76037886797324\\
88.4848484848485	5.76037886797324\\
90.9090909090909	5.76037886797324\\
93.3333333333333	5.76037886797324\\
95.7575757575758	5.76037886797324\\
98.1818181818182	5.76037886797324\\
100.606060606061	5.76037886797324\\
103.030303030303	5.76037886797324\\
105.454545454545	5.76037886797324\\
107.878787878788	5.76037886797324\\
110.30303030303	5.76037886797324\\
112.727272727273	5.76037886797324\\
115.151515151515	5.76037886797324\\
117.575757575758	5.76037886797324\\
120	5.76037886797324\\
};
\addplot[only marks, mark=*, mark options={}, mark size=3.0000pt, draw=red, fill=red, forget plot] table[row sep=crcr]{%
x	y\\
-120	21.2755108219021\\
-100	14.6393513337019\\
-80	6.20222108445047\\
-60	3.12848947028955\\
-40	0.917188696120813\\
-20	0.277376714029505\\
20	-0.490626184085273\\
40	-0.447488203921784\\
60	-0.00963412770488054\\
80	1.35996065063824\\
100	5.4517376329768\\
120	16.8204585272815\\
};
\end{axis}

\begin{axis}[%
width=7.250in,
height=1.400in,
at={(1.213in,2.000in)},
scale only axis,
xmin=-120,
xmax=120,
xtick={-120, -80, -40, 0, 40, 80, 120},
xticklabels={},
ymin=-10,
ymax=10,
ytick={-10, 0, 10},
ylabel style={font=\color{white}},
ylabel={\Huge $\bar{\xi}^b_y$ (mm/s)},
axis background/.style={fill=white},
every tick label/.append style={font=\LARGE},
xticklabel style={yshift=-4pt},
yticklabel style={xshift=-3pt},
xtick pos=left,
ytick pos=left,
%axis x line*=bottom,
%axis y line*=left,
%xmajorgrids,
%ymajorgrids
]
\addplot [color=blue, forget plot, line width=2.0pt]
  table[row sep=crcr]{%
-120	0.797324019013954\\
-117.575757575758	0.797324019013954\\
-115.151515151515	0.797324019013954\\
-112.727272727273	0.797324019013954\\
-110.30303030303	0.797324019013954\\
-107.878787878788	0.797324019013954\\
-105.454545454545	0.797324019013954\\
-103.030303030303	0.797324019013954\\
-100.606060606061	0.797324019013954\\
-98.1818181818182	0.797324019013954\\
-95.7575757575758	0.797324019013954\\
-93.3333333333333	0.797324019013954\\
-90.9090909090909	0.797324019013954\\
-88.4848484848485	0.797324019013954\\
-86.0606060606061	0.797324019013954\\
-83.6363636363636	0.797324019013954\\
-81.2121212121212	0.797324019013954\\
-78.7878787878788	0.797324019013954\\
-76.3636363636364	0.797324019013954\\
-73.9393939393939	0.797324019013954\\
-71.5151515151515	0.797324019013954\\
-69.0909090909091	0.797324019013954\\
-66.6666666666667	0.797324019013954\\
-64.2424242424242	0.797324019013954\\
-61.8181818181818	0.797324019013954\\
-59.3939393939394	0.797324019013954\\
-56.969696969697	0.797324019013954\\
-54.5454545454545	0.797324019013954\\
-52.1212121212121	0.797324019013954\\
-49.6969696969697	0.797324019013954\\
-47.2727272727273	0.797324019013954\\
-44.8484848484849	0.797324019013954\\
-42.4242424242424	0.797324019013954\\
-40	0.797324019013954\\
-37.5757575757576	0.797324019013954\\
-35.1515151515151	0.797324019013954\\
-32.7272727272727	0.797324019013954\\
-30.3030303030303	0.797324019013954\\
-27.8787878787879	0.797324019013954\\
-25.4545454545455	0.797324019013954\\
-23.030303030303	0.797324019013954\\
-20.6060606060606	0.797324019013954\\
-18.1818181818182	0.797324019013954\\
-15.7575757575758	0.797324019013954\\
-13.3333333333333	0.797324019013954\\
-10.9090909090909	0.797324019013954\\
-8.48484848484848	0.797324019013954\\
-6.06060606060606	0.797324019013954\\
-3.63636363636364	0.797324019013954\\
-1.21212121212121	0.797324019013954\\
1.21212121212121	0.797324019013954\\
3.63636363636364	0.797324019013954\\
6.06060606060606	0.797324019013954\\
8.48484848484848	0.797324019013954\\
10.9090909090909	0.797324019013954\\
13.3333333333333	0.797324019013954\\
15.7575757575758	0.797324019013954\\
18.1818181818182	0.797324019013954\\
20.6060606060606	0.797324019013954\\
23.030303030303	0.797324019013954\\
25.4545454545455	0.797324019013954\\
27.8787878787879	0.797324019013954\\
30.3030303030303	0.797324019013954\\
32.7272727272727	0.797324019013954\\
35.1515151515151	0.797324019013954\\
37.5757575757576	0.797324019013954\\
40	0.797324019013954\\
42.4242424242424	0.797324019013954\\
44.8484848484849	0.797324019013954\\
47.2727272727273	0.797324019013954\\
49.6969696969697	0.797324019013954\\
52.1212121212121	0.797324019013954\\
54.5454545454545	0.797324019013954\\
56.969696969697	0.797324019013954\\
59.3939393939394	0.797324019013954\\
61.8181818181818	0.797324019013954\\
64.2424242424242	0.797324019013954\\
66.6666666666667	0.797324019013954\\
69.0909090909091	0.797324019013954\\
71.5151515151515	0.797324019013954\\
73.9393939393939	0.797324019013954\\
76.3636363636364	0.797324019013954\\
78.7878787878788	0.797324019013954\\
81.2121212121212	0.797324019013954\\
83.6363636363636	0.797324019013954\\
86.0606060606061	0.797324019013954\\
88.4848484848485	0.797324019013954\\
90.9090909090909	0.797324019013954\\
93.3333333333333	0.797324019013954\\
95.7575757575758	0.797324019013954\\
98.1818181818182	0.797324019013954\\
100.606060606061	0.797324019013954\\
103.030303030303	0.797324019013954\\
105.454545454545	0.797324019013954\\
107.878787878788	0.797324019013954\\
110.30303030303	0.797324019013954\\
112.727272727273	0.797324019013954\\
115.151515151515	0.797324019013954\\
117.575757575758	0.797324019013954\\
120	0.797324019013954\\
};
\addplot[only marks, mark=*, mark options={}, mark size=3.0000pt, draw=red, fill=red, forget plot] table[row sep=crcr]{%
x	y\\
-120	-4.86569419063302\\
-100	-4.87975157374232\\
-80	-5.58108042372111\\
-60	-4.01219246436612\\
-40	-2.10969748167624\\
-20	-1.18060456327746\\
20	1.84171869184155\\
40	4.68582356452843\\
60	6.19804964648133\\
80	4.99981049179915\\
100	7.93984138806012\\
120	6.53166514287312\\
};
\end{axis}

\begin{axis}[%
width=7.250in,
height=1.400in,
at={(1.213in,0.200in)},
scale only axis,
xmin=-120,
xmax=120,
xtick={-120, -80, -40, 0, 40, 80, 120},
xlabel style={font=\color{white!15!black}},
xlabel={\Huge $\bar{A}$ (mm)},
ymin=-10,
ymax=10,
ytick={-10, 0, 10},
ylabel style={font=\color{white}},
ylabel={\Huge $\bar{\xi}^b_\omega$ (deg/s)},
axis background/.style={fill=white},
every tick label/.append style={font=\LARGE},
xticklabel style={yshift=-4pt},
yticklabel style={xshift=-3pt},
xtick pos=left,
ytick pos=left,
%axis x line*=bottom,
%axis y line*=left,
%xmajorgrids,
%ymajorgrids
]
\addplot [color=blue, forget plot, line width=2.0pt]
  table[row sep=crcr]{%
-120	-5.20285999460052\\
-117.575757575758	-5.10018381577648\\
-115.151515151515	-4.99750763695243\\
-112.727272727273	-4.89483145812839\\
-110.30303030303	-4.79215527930435\\
-107.878787878788	-4.6894791004803\\
-105.454545454545	-4.58680292165626\\
-103.030303030303	-4.48412674283222\\
-100.606060606061	-4.38145056400817\\
-98.1818181818182	-4.27877438518413\\
-95.7575757575758	-4.17609820636009\\
-93.3333333333333	-4.07342202753604\\
-90.9090909090909	-3.970745848712\\
-88.4848484848485	-3.86806966988796\\
-86.0606060606061	-3.76539349106391\\
-83.6363636363636	-3.66271731223987\\
-81.2121212121212	-3.56004113341583\\
-78.7878787878788	-3.45736495459179\\
-76.3636363636364	-3.35468877576774\\
-73.9393939393939	-3.2520125969437\\
-71.5151515151515	-3.14933641811966\\
-69.0909090909091	-3.04666023929561\\
-66.6666666666667	-2.94398406047157\\
-64.2424242424242	-2.84130788164753\\
-61.8181818181818	-2.73863170282348\\
-59.3939393939394	-2.63595552399944\\
-56.969696969697	-2.5332793451754\\
-54.5454545454545	-2.43060316635136\\
-52.1212121212121	-2.32792698752731\\
-49.6969696969697	-2.22525080870327\\
-47.2727272727273	-2.12257462987923\\
-44.8484848484849	-2.01989845105518\\
-42.4242424242424	-1.91722227223114\\
-40	-1.8145460934071\\
-37.5757575757576	-1.71186991458305\\
-35.1515151515151	-1.60919373575901\\
-32.7272727272727	-1.50651755693497\\
-30.3030303030303	-1.40384137811092\\
-27.8787878787879	-1.30116519928688\\
-25.4545454545455	-1.19848902046284\\
-23.030303030303	-1.09581284163879\\
-20.6060606060606	-0.993136662814752\\
-18.1818181818182	-0.890460483990709\\
-15.7575757575758	-0.787784305166666\\
-13.3333333333333	-0.685108126342623\\
-10.9090909090909	-0.58243194751858\\
-8.48484848484848	-0.479755768694537\\
-6.06060606060606	-0.377079589870494\\
-3.63636363636364	-0.274403411046451\\
-1.21212121212121	-0.171727232222407\\
1.21212121212121	-0.0690510533983644\\
3.63636363636364	0.0336251254256787\\
6.06060606060606	0.136301304249722\\
8.48484848484848	0.238977483073765\\
10.9090909090909	0.341653661897808\\
13.3333333333333	0.444329840721851\\
15.7575757575758	0.547006019545894\\
18.1818181818182	0.649682198369937\\
20.6060606060606	0.75235837719398\\
23.030303030303	0.855034556018023\\
25.4545454545455	0.957710734842066\\
27.8787878787879	1.06038691366611\\
30.3030303030303	1.16306309249015\\
32.7272727272727	1.2657392713142\\
35.1515151515151	1.36841545013824\\
37.5757575757576	1.47109162896228\\
40	1.57376780778632\\
42.4242424242424	1.67644398661037\\
44.8484848484849	1.77912016543441\\
47.2727272727273	1.88179634425845\\
49.6969696969697	1.9844725230825\\
52.1212121212121	2.08714870190654\\
54.5454545454545	2.18982488073058\\
56.969696969697	2.29250105955463\\
59.3939393939394	2.39517723837867\\
61.8181818181818	2.49785341720271\\
64.2424242424242	2.60052959602676\\
66.6666666666667	2.7032057748508\\
69.0909090909091	2.80588195367484\\
71.5151515151515	2.90855813249888\\
73.9393939393939	3.01123431132293\\
76.3636363636364	3.11391049014697\\
78.7878787878788	3.21658666897101\\
81.2121212121212	3.31926284779506\\
83.6363636363636	3.4219390266191\\
86.0606060606061	3.52461520544314\\
88.4848484848485	3.62729138426719\\
90.9090909090909	3.72996756309123\\
93.3333333333333	3.83264374191527\\
95.7575757575758	3.93531992073932\\
98.1818181818182	4.03799609956336\\
100.606060606061	4.1406722783874\\
103.030303030303	4.24334845721144\\
105.454545454545	4.34602463603549\\
107.878787878788	4.44870081485953\\
110.30303030303	4.55137699368357\\
112.727272727273	4.65405317250762\\
115.151515151515	4.75672935133166\\
117.575757575758	4.8594055301557\\
120	4.96208170897975\\
};
\addplot[only marks, mark=*, mark options={}, mark size=3.0000pt, draw=red, fill=red, forget plot] table[row sep=crcr]{%
x	y\\
-120	-6.00724494350607\\
-100	-4.08016984100807\\
-80	-3.08598150458782\\
-60	-2.21254753191912\\
-40	-1.58500614184543\\
-20	-0.709215297195201\\
20	0.47865530683246\\
40	1.24772101888134\\
60	2.03575070121263\\
80	2.74586645114967\\
100	3.56666021916837\\
120	6.1608418490926\\
};
\end{axis}
\end{tikzpicture}%

